Fully Dynamic Almost-Maximal Matching: Breaking the Polynomial Barrier for Worst-Case Time Bounds

Despite significant research efforts, the state-of-the-art algorithm for maintaining an approximate matching in fully dynamic graphs has a polynomial {worst-case} update time, even for very poor approximation guarantees. In a recent breakthrough, Bhattacharya, Henzinger and Nanongkai showed how to maintain a constant approximation to the minimum vertex cover, and thus also a constant-factor estimate of the maximum matching size, with polylogarithmic worst-case update time. Later (in SODA'17 Proc.) they improved the approximation factor all the way to $2+\epsilon$. Nevertheless, the longstanding fundamental problem of {maintaining} an approximate matching with sub-polynomial worst-case time bounds remained open. We present a randomized algorithm for maintaining an {almost-maximal} matching in fully dynamic graphs with polylogarithmic worst-case update time. Such a matching provides $(2+\epsilon)$-approximations for both the maximum matching and the minimum vertex cover, for any $\epsilon > 0$. Our result was done independently of the $(2+\epsilon)$-approximation result of Bhattacharya et al., so it provides the first $(2+\epsilon)$-approximation for minimum vertex cover (together with Bhattacharya et al.'s result) and the first $(2+\epsilon)$-approximation for maximum (integral) matching. The polylogarithmic worst-case update time of our algorithm holds deterministically, while the almost-maximality guarantee holds with high probability. This result not only settles the aforementioned problem on dynamic matchings, but also provides essentially the best possible approximation guarantee for dynamic vertex cover (assuming the unique games conjecture).

==> BHN.tex <==
\section{Obtaining $(3+\eps)$-approximate matching} \label{3+eps}
The SODA'17 paper of \cite{BHN17} maintains a $(2+\epsilon)$-approximate fractional matching in $O(\log^3 n)$ worst-case update time.
In order to maintain a $(3+\eps)$-approximate integral matching, one can sample the edges with probabilities proportional to $\log n$ times their fractional edge-weights in the \cite{BHN17} paper, and then reset the weight of every sampled edge to $\log n$. The sampled edges form a subgraph of maximum degree $O(\poly(\log n,\eps^{-1}))$, and furthermore, this subgraph should contain a fractional matching whose size is the same as the size of the fractional matching maintained by the \cite{BHN17} paper to within a factor of $1+\eps$.
Since the maximum degree in this subgraph is bounded by $O(\poly(\log n,\eps^{-1}))$, one can maintain a $(1+\epsilon)$-approximate integral matching in this subgraph using the algorithm by \cite{GP13} with $O(\poly(\log n,\eps^{-1}))$ worst-case update time,
but this transition from a fractional matching to an integral one incurs a loss of multiplicative factor of $3/2$ to the approximation guarantee in general graphs.
Since the fractional matching maintained by \cite{BHN17} has an approximation guarantee of $2+\epsilon$,
this method should give rise to a randomized algorithm for maintaining a $(2+\epsilon) \cdot (3/2 + \epsilon) = (3+\epsilon)$-approximate matching with a worst-case update time of $O(\poly(\log n,\eps^{-1}))$, in the oblivious adversarial model.

Although we do not see a flaw with this argument, we did not make an effort to verify its correctness.
If correct, it shows that given  the \cite{BHN17} algorithm as a black box, it is not difficult to maintain a $(3+\epsilon)$-approximate (integral) matching with $O(\poly(\log n,\eps^{-1}))$ worst-case update time using a randomized algorithm.
The drawback of this approach is that the algorithm of \cite{BHN17} is quite complex.

As mentioned, our result was done independently to the SODA'17 paper of \cite{BHN17}, and it leads to a $(2+\eps)$-approximation on the maintained matching (rather than  $(3+\eps)$-approximation), thus resolving Question 1 in the affirmative.
(When it comes to approximate matching and vertex cover, there is a very significant difference between a $(2+\eps)$-approximation and a $(3+\eps)$-approximation.) 

==> almost-maximality.tex <==
\section{Proof of (Almost-)Maximality} \label{sec:almost}
%[[S: should rename the title of this section, and rewrite the entire section according to the notation I use]]
%\subsection{Some observations}
To prove that the matching is always almost-maximal,
we need to show that the number of temporarily free vertices at any point in time is just an $\eps$-fraction of the number of matched edges.


At any point in time, at most $O(\log n)$ threads are running.
Each of these threads may cause only $O(1)$ vertices to become temporarily free throughout its execution.
(This assertion holds trivially for all threads, except for those that run Procedure $\evalf$, but for those the assertion follows from Corollary \ref{boundactive}.)
Moreover, by the time any such thread terminates its execution, none of these vertices remains temporarily free, i.e., some of these vertices become matched
while the others become free.
It follows that the update algorithm causes only $O(\log n)$ vertices to be temporarily free at any point in time,
and all these vertices are being taken care of by appropriate threads of the algorithm.

As shown in Section \ref{app:small}, one can maintain a maximal matching easily and efficiently when the matching size is small,
and   we may henceforth assume that the matching is sufficiently large. (A formal case analysis is provided after Lemma \ref{whp}.)
''Losing'' $O(\log n)$ vertices due to the update algorithm is thus negligible, % whenever the matching size is $\Omega(\log n /\eps)$.
%The challenging part is to copre with large matchings.
%In particular, assuming the matching is of , losing $O(\log n)$ vertices is negligible.
and our challenge is to bound the number of temporarily free vertices due to the adversary.

Consider first temporarily free vertices at levels $\ell$ with $T_\ell / \Delta < 1$.
Note that the simulation time of a level-$\ell$ thread is either $T_\ell / \Delta$ or $T_\ell / \Delta'$, and so
%where $T_\ell / \Delta := \Theta(\eps(\gamma^\ell /\log n))$
the number of update operations needed for simulating the execution of any level-$\ell$ thread is smaller than 1.
%First, note that for any level $\ell$ such that , we have $T_\ell /\Delta = O(\eps(2^\ell / \log n)) < 1$.
Thus any of the level-$\ell$ threads finishes its execution without simulating it over subsequent update operations, which means that
following an adversarial edge deletion that deletes a matched edge $(u,v)$, the relevant thread
(which executes the   calls $\evalf(u)$ and $\evalf(v)$) terminates its execution before the adversary  makes the next edge deletion.
Thus there are no temporarily free vertices due to the adversary at any such level.   % $\ell$ for which $2^\ell = o(\log n / \eps)$.

Next, we consider temporarily free vertices at the remaining levels, i.e., with $T_\ell / \Delta \ge 1$.
For any such level, Invariant \ref{samp:in} holds,
thus the samples of all level-$\ell$ edges always contain at least $(1-2\eps) \cdot \gamma^{\ell}$ edges.
\vspace{7pt}
\\
\noindent
{\bf The offline model.~}
For levels with $T_\ell / \Delta \ge 1$, all   samples are almost full, so the adversary will not delete any matched edge throughout the entire update sequence.
Thus all $\log_\gamma(n-1) + 1$ queues $Q_0,Q_1,\ldots,Q_{\log_{\gamma}(n-1)}$ of temporarily free vertices are always    empty,
and at any time all $O(\log n)$ vertices that are currently temporarily free are being taken care of by appropriate threads of the algorithm.
Assuming the matching is of size at least $\Omega(\log n / \eps)$, it must be  almost-maximal (deterministically).
\vspace{7pt}
\\
\noindent
{\bf The standard oblivious adversarial model.~}
In what follows we consider the oblivious adversarial model, and show that the adversary is not likely to cause too many vertices to become temporarily free.  % matched edges from the graph.
As explained in Section \ref{short:app}, we may assume that the length of the update sequence is $O(n^2)$.

Any matched edge is created by the algorithm by first determining its level, and only then performing the   sampling.
If the edge is matched at level $\ell$,  it is chosen uniformly at random from  between $(1-\eps) \cdot \gamma^{\ell}$ and $\gamma^{\ell}$ edges.
%Fix an arbitrary level for which $T_\ell / \Delta \ge 1$.
% and note that any matched edge at level $\ell$
%Note that the random sampling that is carried out for creating any matched edge at level-$\ell$ is performed after determining its level $\ell$.
We   thus  fix some level $\ell$ with $T_\ell / \Delta \ge 1$, and focus on the matched edges at that level.

Consider any time step $t$, and let $V_t$ be the set of vertices at level $\ell$ at time $t$, excluding vertices that are temporarily free due to the update algorithm.
Let $A_t = A'_t \cap A''_t$,
where $A'_t$ is the event that $|V_t|  \ge c'(\log^4 n /\eps^3)$,
%(\log^4 n /\eps^2)$
$A''_t$ is the event that at least a $(c''\cdot \eps)$-fraction of the vertices of $V_t$ are temporarily free due to the adversary at time $t$,
and $c'$ and $c''$ are sufficiently large constants.  % with $c' \gg c'' \gg 1$.
%among all epochs that are present at time $t$ (i.e., those that have not been replaced by the scheduler),
%Our goal is to show that $E_t$ occurs with low probability, or formally:
The following lemma is central in our proof of the almost-maxiamlity guarantee, and its proof is provided in Sections \ref{highlight}--\ref{cont}.
Then in Section \ref{conclude} we derive the almost-maximality guarantee as a corollary of this lemma.
% the proof of this lemma employs the shuffling game described in Section \ref{shuffling}. %; some details are sketched below, the full proof is given in Section
\begin{lemma} \label{whp}
$\Prob(A_t) = O(n^{-c+2})$, for some constant $c$ that depends on $c'$ and $c''$.
\end{lemma}
\subsection{Proof of Lemma \ref{whp}, part I: Overview and challenges} \label{highlight}
%\begin{proof}
%The proof of this lemma is technically involved, and provided in the following section.
%\subsection{Proof of Lemma \ref{whp}} \label{techs}
%We start with a high-level overview with the proof.
%In Section \ref{shuffling} we describe and analyze the a certain game, which we refer to as the \emph{shuffling game}.
%Equipped with the result for the shuffling game, in App.\ \ref{cont} we provide the proof of Lemma \ref{whp}.  %, which employs the result for the shuffling game.
%\subsection
%\subsubsection{Proof highlights}
Any matched edge is sampled uniformly at random from between $(1-\eps) \cdot \gamma^{\ell}$ and $\gamma^{\ell}$ edges.
Since the samples of all level-$\ell$ edges always contain $\ge (1-2\eps) \cdot \gamma^{\ell}$ edges,
at the moment a matched edge is created at level $\ell$, its probability of getting deleted by the adversary while it is matched (hereafter, getting \emph{hit})
is $\le 2\eps$. %Intuitively, as time goes by and as long as this matched edge does not get hit, its probability of getting hit may only decrease. 
Our argument, alas, is not applied on all matched edges created since the algorithm's outset, but rather on a subset of edges that are matched at a certain time step $t'$,
and there are dependencies on previous coin flips of our algorithm, which are the result of edges being deleted from the matching by the update algorithm itself (not the adversary).
%the fact that an edge remains matched until a certain time step $t'$ may reveal information on coin flips made by our algorithm at previous time steps, and
Indeed, given that some edge $e$ is matched at time $t'$, the sample of $e$ may be significantly reduced,
%(a-priori, all edges in the sample but $e$ may get deleted by the algorithm prior to time $t'$ with probability 1), %potentially to consist of just that particular edge,
which could increase the probability of $e$ getting hit.
%To clarify, this issue arises due to deletions of edges from the matching by the update algorithm.
%A-priori, it could be that

For a matched edge $e$, consider the edges of its sample $S^*(e)$ in the order they are deleted by the adversary, 
even after the edge is removed from the matching, either by the adversary or by the algorithm.
A matched edge is called \emph{bad} if it is one of the first (at most) $2\eps \cdot \gamma^{\ell}$ edges in this ordering; otherwise it is good.
Since at most $2\eps \cdot \gamma^{\ell}$ edges are removed from the sample of each matched edge (while it is matched), 
%there is an adversarial deletion of that edge after the time it got matched; otherwise it is good.
a good edge cannot get hit;
%may only get deleted from the matching by the algorithm;   % and it will remain matched throughout otherwise;
a bad edge gets hit, unless it is deleted from the matching by the algorithm prior to the corresponding adversarial deletion of that edge.
To overcome the aforementioned  hurdle, we use  $\shuffle$ to show that the fraction of bad edges at any point in time is $O(\eps)$.
To this end, we apply a game, hereafter the \emph{shuffling game},  %, described and analyzed in detail in Section \ref{shuffling}.
where in each step a single edge is either added or deleted (starting with no edges) by the following players:
(1) $\adder$: adds an edge, which is bad w.p.\ $\le 2\eps$, (2) $\shuf$: deletes an edge uniformly at random among the existing edges,
(3) $\mal$: deletes a good edge.
A newly created matched edge is bad w.p.\ $\le 2\eps$, thus $\adder$ assumes the role of creating matched edges by the algorithm,
and so an $O(\eps)$-fraction of the matched edges created by $\adder$ are bad w.h.p.
(In this overview we assume that the number of edges added and deleted is sufficiently large to obtain high probability bounds,
but this assumption is formally justified in Section  \ref{justify}.)
$\shuf$ assumes the role of $\shuffle$ in the algorithm, deleting matched edges uniformly at random.
If the fraction of bad edges during some time interval is $\Theta(\eps)$, the fraction of bad edges deleted by $\shuf$ in this interval is $\Theta(\eps)$ w.h.p.,
hence $\shuf$ does not change the fraction of bad edges by too much.
The role of $\mal$ is not to model the exact behavior of the other (non-shuffled) parts of the algorithm that delete matched edges, but rather to capture the worst-case scenario that might happen. We show that even if the other (non-shuffled) parts were to delete only good edges, the fraction of bad edges would be $O(\eps)$, just as if $\mal$ were not in the game.
Specifically, we prove that the fraction of bad edges at any time step $t'$ is w.h.p.\ $O(\eps)$.
This proof, provided in Section \ref{shuffling}, is nontrivial and makes critical use of the fact (see Lemma \ref{faster}) that $\shuf$ is faster than $\mal$ by a logarithmic factor.

%although intuitively obvious, the proof for this assert ion is nontrivial.


Equipped with this bound on the fraction of bad edges at any time step,
% $t'$ is the last time step until $t$ where the queue $Q^{(t')}_\ell$ was empty
we consider the last time   $t'$ prior to $t$ in which the queue $Q_\ell$ of temporarily free level-$\ell$ vertices is empty, i.e., $Q_\ell$ is non-empty in the entire time interval $[t'+1,t]$, which means that $\temp_\ell$ is never idle during that time.
We need to bound the fraction of bad edges not only among the ones matched at time $t'$, but also among those that get matched between times $t'$ and $t$.
The fraction of bad edges among those matched at time $t'$ is $O(\eps)$ w.h.p.\ by the shuffling game; as for
those that get created later on, there is no dependency on coin flips that the algorithm made prior to time $t'$, and so the probability of any of those edges to
be bad is $\le 2\eps$, independently of whether previously created matched edges are bad, and by Chernoff we get that the fraction of bad edges among them is also $O(\eps)$ w.h.p.
The formal proof for this bound on the fraction of bad edges among those is provided in Section \ref{cont}, and it implies that only an $O(\eps)$-fraction of   those edges may get hit w.h.p., and thus get into the queue.
This bound, however, does not suffice to argue that the number of  vertices in $Q_\ell$ at time $t$ is an $O(\eps)$-fraction of the matching size, due to edges that get deleted from the matching by the algorithm itself. Since $\temp_\ell$ is no slower than the other sub-schedulers (as its simulation parameter is $\Delta'$),
we show in Section \ref{cont} that it removes vertices from $Q_\ell$ in the interval $[t'+1,t]$ at least at the same (up to a constant) rate   as  matched edges get deleted by the algorithm.
By formalizing  these assertions and carefully combining them, we conclude with the required result.

\input{shufflingGamev3}

\input{pf-lemma-whp}
%\input{shuffle}

\subsection{Corollaries of Lemma \ref{whp}: The almost-maximality guarantee and main results} \label{conclude}


%{\bf Remark.} The constant $c$ depends on several constants, including: (1) The constant hidden in the $\Omega$-notation in the statement of this lemma.
%(2) The leading constant 10 (i.e., the $10\eps$-fraction) in the definition of the event $E_t$. (3) The upper bound on the maximum number of edges deleted from any epoch, %guaranteed by the scheduler. (We may want to try optimizing these constants, probably not...)
%\vspace{5pt}
Applying a union bound over all $O(n^2)$ time steps and over all levels,  % where $E = \Omega(\log n/\eps)$,
we conclude that  at any point in time, with probability at most $O(n^{-c+4} \cdot \log n) = O(n^{-c+5})$,
%, disregarding the matched edges at levels which we ignore,
an $\Omega(\eps)$-fraction of the potential matched vertices at all levels where there are at least $\Omega(\log^4 n /\eps^3)$ vertices are unmatched.
At any level that we ignore, we may lose at most $O(\log^4 n /\eps^3)$ potential matched vertices by definition.
Whenever the size of the maximum matching is $\Omega(\log^5 n /\eps^4)$,
the loss due to the levels that we ignore is negligible, as those levels contain together just an $O(\eps)$-fraction of the potential matched vertices.
Note also  that we disregarded vertices that are temporarily free due to the update algorithm, but the loss due to those vertices is negligible,
as their total number over all levels is bounded by $O(\log n)$.   % at any point in time.
%In App.\
%they contain another $O(\eps)$-fraction of the potential matched vertices.

Recall that the worst-case update time of our algorithm is $O(\Delta' \cdot \log n) = O(\log^7 n / \eps)$; denote the matching maintained by this algorithm by $\cM_{rand}$.
%and our matching is with probability  at least $1 - O(n^{-c+5})$ ``almost-maximal'', i.e., we never lose more than an $O(\eps)$-fraction of the potential matched vertices.
%Consider next the case where the maximal matching $\cM$ is of size $O((\log n /\eps)^2)$.
Set $\delta = \Theta(\log^5 n /\eps^4)$.
As explained above, $\cM_{rand}$ is guaranteed to be almost-maximal w.h.p.\ whenever the maximum matching size is no smaller than $\delta$.
As explained in Section \ref{app:small}, one can   maintain a   matching $\cM_\delta$ with a worst-case update time of $O(\log^5 n /\eps^4)$,
which is guaranteed to be   maximal whenever  $|\cM_\delta| < \delta$, which must hold when the maximum matching size is smaller than $\delta$.
%(The algorithm maintaining this matching is applied regardless of the matching size, but
%the strict maximality guarantee holds only whenever $\cM = O((\log n /\eps)^2)$.)
Therefore, we maintain these two matchings $\cM_{rand}$ and $\cM_{\delta}$  throughout the update sequence,
%We will maintain two matchings with a worst-case update time of $\max\{O((\log n /\eps)^2),O((\log^5 n) / \eps)\}$, one via the algorithm above, denoted $\cM_{\delta}$,
%and another via the randomized algorithm, denoted $\cM_{rand}$.
%Whenever $|\cM_{\delta}| < \delta$, Lemma \ref{maxdelta} guarantees that $\cM_{\delta}$ is maximal.
%In the complementary regime $|\cM_{\delta}| \ge \delta$, the size of the maximum matching $\cM^*$ is at least $\delta$,
%and then $\cM_{rand}$ is guaranteed to be almost-maximal w.h.p.
and at any point in time return $\cM_{\delta}$ as the output matching if $|\cM_{\delta}| < \delta$ and $\cM_{rand}$ otherwise.
%Therefore, if the size of the maximal matching $\cM$ is $O((\log n /\eps)^2)$, we maintain an exact maximal matching with a worst-case update time of $O((\log n /\eps)^2)$.

Summarizing, a worst-case update time of $O(\max\{\log^7 n /\eps,\log^5 n / \eps^4\})$ suffices to maintain a $(1-\eps)$-almost-maximal matching with probability at least $1 - O(n^{-c+5})$ at any point in time (where we never lose more than an $O(\eps)$-fraction of the potential matched vertices).
\begin{theorem} [standard oblivious adversarial model] \label{maint}
Let $\eps \ll 1$ be an arbitrary parameter.
Starting from an empty graph on $n$ fixed vertices, an $(1-\eps)$-maximal matching (and thus a $(2+\eps)$-approximation for both the maximum matching and the minimum vertex cover) can be maintained over any
sequence of edge updates with a (deterministic) worst-case update time of $O(\max\{\log^7 n /\eps,\log^5 n / \eps^4\})$, where the almost-maximality guarantee $1-\eps$ holds both in expectation and w.h.p.
\end{theorem}
{\bf Remarks.}
~(1) The argument above does not bound the expected almost-maximality guarantee directly,
but an expected bound is   implied by the definition of expectation, following similar lines as in the proof of Lemma \ref{whp}.
On the other hand, an expected bound would not yield our high probability guarantee.
\vspace{5pt}
\\
~(2) Note that the output matching may change significantly following a single edge update,
since $\cM_{\delta}$ and $\cM_{rand}$ may be very different. We can strengthen the result to make sure that the number of changes (replacements) to the output matching
is linear in the worst-case update time of the algorithm, by maintaining a $(1+\eps)$-approximate maximum matching
over the union of $\cM_{\delta}$ and $\cM_{rand}$ using a \emph{modified version} of the algorithm of \cite{GP13}.
Specifically, for bounded degree graphs, the worst-case update time of the algorithm of \cite{GP13} is $O(1/\eps^2)$,
but the worst-case number of replacements to the matching maintained by the algorithm of \cite{GP13} may be huge.
Consequently, we first strengthen the algorithm of \cite{GP13} to bound the number of replacements to the matching by $O(1/\eps^2)$ in the worst-case,
and use this stronger version of the algorithm instead of the original version.
This will increase the approximation guarantee to $(2+\eps)(1+\eps)$, which is negligible, and the update time will grow by a factor of $O(1/\eps^2)$.
(See Sections \ref{b11}, \ref{b21} and \ref{changes} for a detailed argument.)
%[[S: may need to add a remark somewhere that the high probability bound holds for any point in time but not to all points in time  simultaneously.
%(Previous works also suffer from this natural disadvantage.)]]
%{\bf Remark.}
\vspace{5pt}
\\
~(3) While the worst-case update time in Theorem \ref{maint} holds deterministically, the almost-maximality guarantee is probabilistic.
Using a symmetric argument, we can ensure that the almost-maximality guarantee holds deterministically, but then the bound on the worst-case update time will be probabilistic.
%{\bf Remarks.}

\vspace{6pt}
Consider next the offline model, where in any point in time and for any subset $E_v$ of edges adjacent to any vertex $v$ ($E_v$ need not contain all edges adjacent to $v$),
we can find in time linear in $E_v$ an edge from $E_v$ that will be deleted from the graph after a constant fraction of the edges of $E_v$ have been deleted.
For the offline setting, our algorithm is deterministic. In particular, there is no reason to maintain the matching
$\cM_{\delta}$, thus shaving the second term ($\log^5 n / \eps^4$) from the update time bound.
Also, as there is no need to use $\shuffle$ for the offline setting,
which works faster than the other schedulers by a logarithmic factor, this shaves a logarithmic factor from the update time immediately.
\begin{theorem} [offline model]
Let $\eps \ll 1$ be an arbitrary parameter. In the offline model,
starting from an empty graph on $n$ fixed vertices, an $(1-\eps)$-maximal matching (and thus a $(2+\eps)$-approximation for both the maximum matching and the minimum vertex cover) can be maintained deterministically over any sequence of edge updates with a worst-case update time of $O(\log^6 n /\eps)$.
\end{theorem}
%tradeoff between the update time and the almost-maximal guarantee
%
% smaller than that, then
%[[S: The durations of epochs are truly independent? That is, we should be able to apply the Chernoff bound?
%We are not writing there $\Prob(E | E') = \Prob(E)$, as this of course says that $E$ and $E'$ are independent, and this should work also in the symmetric way.
%We are saying something like $\Prob(E | E')$ is small enough. But if I know that the duration of some later guy is small, it may reveal some info about me...]]
%\vspace{0pt}
%\\
%\noindent


==> pdfpages.tex <==
%%
%% This is file `pdfpages.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% pdfpages.dtx  (with options: `package')
%%
%% This is a package for PDFLaTeX, which makes it
%% easy to insert pages of external PDF documents.
%%
%% This file is part of the pdfpages package.
%%
%% Copyright (C) 2001 2002 Andreas MATTHIAS.
%%
%% This program may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.2
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.2 or later is part of all distributions of LaTeX
%% version 1999/12/01 or later.
%%
%% Please send error reports and suggestions for improvements to
%%   Andreas MATTHIAS <amat@kabsi.at>.
%%
\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{pdfpages}[2002/04/23 v0.2h Insert pages of external PDF documents (AM)]
\def\AM@version{0.2h}
\begingroup
\@ifundefined{pdfoutput}
   {\PackageError{pdfpages}
            {You're either not using pdfLaTeX\MessageBreak
             or have turn off PDF output.\MessageBreak
             `pdfpages' only works with pdfLaTeX\MessageBreak
             and PDF output}
            {Use `pdflatex' instead of `latex'\MessageBreak
             and set output to PDF (use: \pdfoutput = 1)!}
    \endinput}
   {\ifnum\pdfoutput=\z@
      \PackageError{pdfpages}
            {You don't produce PDF output, which\MessageBreak
             is required for the `pdfpages' package}
            {Set output to PDF. (use: \pdfoutput = 1)}
      \expandafter\endinput
    \fi}
\endgroup
\RequirePackage{ifthen, graphicx, calc, eso-pic}
\def\AM@ifdriverlater{\@ifl@ter{def}}
\AM@ifdriverlater{pdftex}{2000/05/12}{}{%
    \PackageError{pdfpages}{%
         You have an old `pdftex.def'.\MessageBreak%
         There is no multipage support\MessageBreak%
         in `pdftex.def' < 0.02u.\MessageBreak%
         Update your `pdftex.def'}
         {Update your `pdftex.def'!}}
\AM@ifdriverlater{pdftex}{2000/09/14}{}{%
    \PackageWarning{pdfpages}{%
         You have an old `pdftex.def'.\MessageBreak%
         There might be problems with\MessageBreak%
         the `trim' and `clip' options.\MessageBreak%
         Update your `pdftex.def'!\MessageBreak}}
\def\AM@ifdriverlater{\@ifl@ter{sty}}
\AM@ifdriverlater{eso-pic}{2001/07/20}
  {\def\AM@AddToShipoutPicture{\AddToShipoutPicture*}%
   \def\AM@ClearShipoutPicture{\relax}}
  {\def\AM@AddToShipoutPicture{\AddToShipoutPicture}%
   \def\AM@ClearShipoutPicture{\ClearShipoutPicture}}
\newcommand*{\AM@draft}{false}
\DeclareOption{draft}{\def\AM@draft{true}}
\DeclareOption{final}{\def\AM@draft{false}}
\ProcessOptions
\newif\ifAM@openright\AM@openrightfalse
\newif\ifAM@frame\AM@framefalse
\newif\ifAM@landscape\AM@landscapefalse
\newif\ifAM@turn\AM@turntrue
\newif\ifAM@thread\AM@threadfalse
\newif\ifAM@link\AM@linkfalse
\newif\ifAM@linktodoc\AM@linktodocfalse
\newif\ifAM@column\AM@columnfalse
\newif\ifAM@columnstrict\AM@columnstrictfalse
\newif\ifAM@noautoscale\AM@noautoscalefalse
\newif\ifAM@fitpaper\AM@fitpaperfalse
\newif\ifAM@doublepages\AM@doublepagesfalse
\newif\ifAM@linkfilename\AM@linkfilenamefalse
\newif\ifAM@signature\AM@signaturefalse
\newif\ifAM@sigrotate\AM@sigrotatefalse
\newif\ifAM@newwindow\AM@newwindowtrue
\newcommand*{\AM@pagestemp}{1}
\newcommand*{\AM@pagecommand}{\thispagestyle{empty}}
\newcommand*{\AM@lscape@rot}{0}
\newcommand*{\AM@threadname}{}\newcommand*{\AM@linkname}{}
\newcommand*{\AM@linkname@option}{}
\newcommand*{\AM@linkfit}{fitr}\newcommand*{\AM@linktodocfit}{/Fit}
\newcommand*{\threadinfodict}{}
\newcommand*{\AM@toclist}{}\newcommand*{\AM@loflist}{}
\newcommand*{\AM@signature}{}
\newif\ifAM@thumbpdf
\newif\ifAM@pdflscape
\newcommand*{\AM@setlscape}{}
\AtBeginDocument{%
  \@ifpackageloaded{thumbpdf}{\AM@thumbpdftrue}{\AM@thumbpdffalse}%
  \@ifpackageloaded{pdflscape}{\AM@pdflscapetrue}{\AM@pdflscapefalse}%
  \ifAM@thumbpdf
    \ifAM@pdflscape
      \def\AM@setlscape{\PLS@Rotate{90}}%
    \else
      \def\AM@setlscape{\pdfpageattr{/Rotate 90}\AM@thumbpdfwarning}%
    \fi
  \else
    \def\AM@setlscape{\pdfpageattr{/Rotate 90}}%
  \fi}
\newif\ifAM@thumbpdfwarning
\newcommand*{\AM@thumbpdfwarning}{%
  \ifAM@thumbpdfwarning\else\global\AM@thumbpdfwarningtrue
  \PackageWarning{pdfpages}{%
    You are using `thumbpdf.sty' but not\MessageBreak
    `pdflscape.sty'. \MessageBreak
    Please insert `pdflscape.sty' in  your document\MessageBreak
    to get a pleasant PDF document with thumbs.\MessageBreak}\fi}
\newif\ifAM@integer
\newcommand{\AM@checkinteger}{}
\def\AM@checkinteger#1{%
  \ifcat _\ifnum9<1#1_\else A\fi
    \AM@integertrue
  \else
    \AM@integerfalse
  \fi
}
\newcommand*{\includepdfset}[1]{%
  \AM@split@options{pdfpages}{#1}%
  \edef\AM@temp{{pdfpages}{\the\@temptokena}}%
  \expandafter\setkeys\AM@temp
}
\newcommand*{\includepdf}[2][]{%
  \begingroup
  \c@totalnumber=0%
  \IfFileExists{#2}{\edef\AM@currentdocname{#2}}
    {\IfFileExists{#2.pdf}{\edef\AM@currentdocname{#2.pdf}}
       {\PackageError{pdfpages}{Cannot find file `#2'}{}}}%
  \def\AM@threadname{\AM@currentdocname}%
  \AM@split@options{pdfpages}{#1}%
  \edef\AM@temp{{pdfpages}{\the\@temptokena}}%
  \expandafter\setkeys\AM@temp
  \expandafter\AM@readlist\expandafter{\AM@pagestemp}%
  \AM@output{#1}%
  \AM@CheckAtEnd
  \endgroup
  \AM@ClearShipoutPicture
}
\newcommand*{\includepdfmerge}[2][]{%
  \begingroup
  \c@totalnumber=0%
  \def\AM@currentdocname{}%
  \AM@readlist{#2}%
  \AM@split@options{pdfpages}{#1}%
  \edef\AM@temp{{pdfpages}{\the\@temptokena}}%
  \expandafter\setkeys\AM@temp
  \AM@output{#1}%
  \AM@CheckAtEnd
  \endgroup
  \AM@ClearShipoutPicture
}
\newcommand{\AM@CheckAtEnd}{%
  \ifx\@empty\AM@toclist\else
    \PackageWarning{pdfpages}{%
         There's something wrong with the entries\MessageBreak
         of `addtotoc'. Not all entries were\MessageBreak
         processed. Check `addtotoc'}%
  \fi
  \ifx\@empty\AM@loflist\else
    \PackageWarning{pdfpages}{%
         There's something wrong with the entries\MessageBreak
         of `addtolist'. Not all entries were\MessageBreak
         processed. Check `addtolist'}%
  \fi
}
\newcommand{\AM@output}[1]{%
  \@ifundefined{AM@xnup}
    {\def\AM@xnup{\@ne}\def\AM@ynup{\@ne}%
     \def\AM@xnupminusi{\z@}\def\AM@ynupminusi{\z@}}{}%
  \@ifundefined{AM@deltax}
    {\def\AM@deltax{-\fboxrule}\def\AM@deltay{-\fboxrule}}{}%
  \@ifundefined{AM@xoffset}
    {\def\AM@xoffset{\z@}\def\AM@yoffset{\z@}}{}%
  \def\AM@xpos{\z@}\def\AM@ypos{\z@}%
  \setkeys{Gin}{draft=\AM@draft}%
  \ifthenelse{\boolean{AM@landscape}}
    {\def\AM@lscape@rot{90}%
     \@ifundefined{AM@shortnupsyntax}{}
       {\let\AM@temp\AM@xnup
        \let\AM@xnup\AM@ynup
        \let\AM@ynup\AM@temp}%
    }{}%
  \AM@setphantom
  \ifx\AM@signature\@empty\AM@filluppagelist
  \else\AM@prepare@signature\AM@signaturetrue\AM@turnfalse\fi
  \@tempcnta=\AM@xnup\relax \advance\@tempcnta\m@ne
  \edef\AM@xnupminusi{\the\@tempcnta}%
  \@tempcnta=\AM@ynup\relax \advance\@tempcnta\m@ne
  \edef\AM@ynupminusi{\the\@tempcnta}%
  \ifthenelse{\boolean{AM@column}%
              \and\not\boolean{AM@columnstrict}}
         {\AM@getlastn{\AM@doclist}{\AM@nup}%
          \edef\AM@lastndocs{\AM@lastnitems}%
          \AM@getlastn{\AM@pagelist}{\AM@nup}%
          \edef\AM@lastnpages{\AM@lastnitems}%
          \AM@resort
          \AM@count{\AM@pagelist}%
          \expandafter\ifx\expandafter\\\AM@pagelist\\%
            \edef\AM@pagelist{\AM@resortedpagelist}%
            \edef\AM@doclist{\AM@resorteddoclist}%
          \else
            \edef\AM@pagelist{\AM@pagelist,\AM@resortedpagelist}%
            \edef\AM@doclist{\AM@doclist,\AM@resorteddoclist}%
          \fi}{}%
  \ifthenelse{\boolean{AM@frame}}
         {\let\AM@fbox\fbox}
         {\let\AM@fbox\relax
          \setlength{\fboxrule}{\z@}}%
  \ifthenelse{\boolean{AM@openright}}
         {\AM@openright}{}%
  \ifthenelse{\boolean{AM@column}}
         {\def\AM@xnupi{\@ne}
          \def\AM@ynupi{\z@}}
         {\def\AM@xnupi{\z@}
          \def\AM@ynupi{\@ne}}%
  \setlength{\fboxsep}{\z@}%
    \AM@readfirst{\AM@pagelist}%
    \edef\AM@page{\the\toks@}%
    \AM@readfirst{\AM@doclist}%
    \edef\AM@docname{\the\toks@}%
    \ifAM@noautoscale
      \def\AM@scale{1}%
    \else
      \AM@isphantom
      \AM@split@options{Gin@noscale}{#1}%
      \setbox\@tempboxa=\hbox{%
        \expandafter\includegraphics\expandafter[\the\@temptokena,
           page=\AM@page, angle=\AM@lscape@rot]{\AM@docname}}%
    \newpage
    \ifthenelse{\boolean{AM@fitpaper}}
      {\setlength{\paperwidth}{\the\wd\@tempboxa}%
       \setlength{\paperheight}{\the\ht\@tempboxa}%
       \setlength{\pdfpagewidth}{\the\wd\@tempboxa}%
       \setlength{\pdfpageheight}{\the\ht\@tempboxa}%
       \@ifundefined{stockwidth}{}{%
         \setlength{\stockwidth}{\paperwidth}%
         \setlength{\stockheight}{\paperheight}%
         \setlength{\trimtop}{0pt}%
         \setlength{\trimedge}{0pt}}%
      }{}%
      \def\AM@xscale{%
        (\paperwidth - \tw@\fboxrule*\AM@xnup
         - \AM@deltax * \AM@xnupminusi) /
        (\AM@xnup * \real{\strip@pt\wd\@tempboxa})
      }%
      \setlength{\@tempdima}{\AM@xscale}%
      \edef\AM@xscale{\strip@pt\@tempdima}%
      \setlength{\@tempdimb}{\ht\@tempboxa + \dp\@tempboxa}%
      \def\AM@yscale{
        (\paperheight - \tw@\fboxrule*\AM@ynup
         - \AM@deltay *\AM@ynupminusi) /
        (\AM@ynup * \real{\strip@pt\@tempdimb})
      }%
      \setlength{\@tempdima}{\AM@yscale}%
      \edef\AM@yscale{\strip@pt\@tempdima}%
      \@tempdima=\AM@xscale\p@
      \@tempdimb=\AM@yscale\p@
      \ifdim\@tempdima<\@tempdimb
        \let\AM@scale\AM@xscale
      \else
        \let\AM@scale\AM@yscale
      \fi
    \fi
    \let\AM@filelist@save\@filelist
    \AM@split@options{Gin}{#1}%
    \setbox\@tempboxa=\hbox{%
      \expandafter\includegraphics\expandafter[\the\@temptokena,
                       page=\AM@page, scale=\AM@scale,
                       angle=\AM@lscape@rot]{\AM@docname}}%
    \let\@filelist\AM@filelist@save
    \setlength{\@tempdimb}{\ht\@tempboxa + \dp\@tempboxa}%
    \def\AM@xmargin{%
      (\paperwidth - (\wd\@tempboxa+\tw@\fboxrule)*\AM@xnup
       - \AM@deltax * \AM@xnupminusi) * \real{.5}%
    }%
    \def\AM@ymargin{%
      (\paperheight - (\@tempdimb+\tw@\fboxrule)*\AM@ynup
       - \AM@deltay * \AM@ynupminusi) * \real{.5}%
    }%
    \setlength{\@tempdima}{\AM@xmargin}%
    \edef\AM@xmargin{\the\@tempdima}%
    \setlength{\@tempdima}{\AM@ymargin}%
    \edef\AM@ymargin{\the\@tempdima}%
    \ifthenelse{\boolean{AM@landscape}}
         {\edef\AM@temp{\AM@xnup}
          \edef\AM@xnup{\AM@ynup}
          \edef\AM@ynup{\AM@temp}}
         {}%
    \ifAM@signature
      \ifAM@landscape\AM@sigrotatefalse\else\AM@sigrotatetrue\fi
    \fi
  \setboolean{AM@endoflist}{false}%
  \whiledo{\not\boolean{AM@endoflist}}{%
    \AM@getfirst{\AM@pagelist}%
      \edef\AM@page{\the\toks@}%
      \AM@isphantom
      \@tempcnta=\AM@page\relax
      \advance\@tempcnta\m@ne
      \edef\AM@page@linktodoc{\the\@tempcnta}%
    \AM@getfirst{\AM@doclist}%
      \edef\AM@docname{\the\toks@}%
      \ifAM@linkfilename
      \else
        \let\AM@linkfilename\AM@docname
      \fi
      \ifx\@empty\AM@linkname@option \edef\AM@linkname{\the\toks@}
      \else \edef\AM@linkname{\AM@linkname@option} \fi
    \ifthenelse{\boolean{AM@column}}
      {\@tempcnta=\AM@ynupi\relax
       \@tempcntb=\AM@ynup\relax
       \advance\@tempcnta\@ne
       \ifnum\@tempcnta>\@tempcntb
         \@tempcnta=\@ne
         \@tempcntb=\AM@xnupi\relax
         \advance\@tempcntb\@ne
         \edef\AM@xnupi{\the\@tempcntb}%
       \fi
       \edef\AM@ynupi{\the\@tempcnta}%
       \@tempcnta=\AM@xnupi\relax
       \@tempcntb=\AM@xnup\relax
       \ifnum\@tempcnta>\@tempcntb
         \def\AM@xnupi{\@ne}%
       \fi
      }
      {\@tempcnta=\AM@xnupi\relax
       \@tempcntb=\AM@xnup\relax
       \advance\@tempcnta\@ne
       \ifnum\@tempcnta>\@tempcntb
         \@tempcnta=\@ne
         \@tempcntb=\AM@ynupi\relax
         \advance\@tempcntb\@ne
         \edef\AM@ynupi{\the\@tempcntb}%
       \fi
       \edef\AM@xnupi{\the\@tempcnta}%

       \@tempcnta=\AM@ynupi\relax
       \@tempcntb=\AM@ynup\relax
       \ifnum\@tempcnta>\@tempcntb
         \def\AM@ynupi{\@ne}%
       \fi
      }%
    \def\AM@add{+}%
    \if@twoside\ifodd\c@page\else\def\AM@add{-}\fi\fi
    \setlength{\@tempdimb}{\ht\@tempboxa + \dp\@tempboxa}%
    \ifthenelse{\boolean{AM@landscape}}
      {\def\AM@xpos{%
         \AM@xmargin \AM@add\AM@xoffset +
         (\wd\@tempboxa + \AM@deltax + \tw@\fboxrule)*(\AM@ynupi - 1)
       }%
       \def\AM@ypos{%
         \AM@ymargin + \AM@yoffset +
         (\@tempdimb + \AM@deltay + \tw@\fboxrule)*(\AM@xnupi - 1)
       }%
      }
      {\def\AM@xpos{%
         \AM@xmargin \AM@add\AM@xoffset +
         (\wd\@tempboxa + \AM@deltax + \tw@\fboxrule)*(\AM@xnupi - 1)
       }%
       \def\AM@ypos{%
         \AM@ymargin + \AM@yoffset +
         (\@tempdimb + \AM@deltay + \tw@\fboxrule)*(\AM@ynup-\AM@ynupi)
       }%
      }%
    \setlength{\@tempdima}{\AM@xpos}%
    \edef\AM@xpos{\strip@pt\@tempdima}%
    \setlength{\@tempdima}{\AM@ypos}%
    \edef\AM@ypos{\strip@pt\@tempdima}%
    \setlength{\fboxsep}{\z@}%
    \ifAM@phantompage
      \def\AM@shippage{}%
    \else
      \AM@split@options{Gin}{#1}%
      \edef\AM@shippage{%
        \noexpand\put(\AM@xpos,\AM@ypos){%
        \noexpand\raisebox{\dp\@tempboxa}{%
        \AM@hyper\noexpand\AM@fbox{%
        \noexpand\includegraphics[\the\@temptokena,
                    page=\AM@page,scale=\AM@scale,
                    \ifAM@sigrotate angle=180\fi,
                    angle=\AM@lscape@rot]{\AM@docname}}}}%
      }%
    \fi
    \AM@AddToShipoutPicture{\setlength{\unitlength}{\p@}%
      \global\let\AM@filelist@save\@filelist}%
    \expandafter\AM@AddToShipoutPicture\expandafter{%
      \AM@shippage
      \global\let\@filelist\AM@filelist@save
    }%
    \AM@toclof{\AM@page}%
    \ifnum\AM@xnupi=\AM@xnup\relax
      \ifnum\AM@ynupi=\AM@ynup\relax
        \begingroup\AM@pagecommand\endgroup
        \hskip\z@
        \ifthenelse{\boolean{AM@turn}}
          {\ifthenelse{\boolean{AM@landscape}}
             {\AM@setlscape}{}}
          {}%
        \newpage
        \ifAM@pdflscape\PLS@Rotate{0}\fi
        \AM@ClearShipoutPicture
        \ifAM@signature
          \ifAM@sigrotate\AM@sigrotatefalse\else\AM@sigrotatetrue\fi
        \fi
      \fi
    \fi
  }% whiledo
}% AM@output
\newif\ifAM@defaultone
\newcommand*{\AM@readlist}[1]{%
  \AM@defaultonefalse
  \def\AM@pagelist{}%
  \def\AM@doclist{}%
  \AM@readlisti#1,\END,
  \ifAM@defaultone\AM@append{1}\fi
  \edef\AM@doclist{\expandafter\@gobble\AM@doclist}%
  \edef\AM@pagelist{\expandafter\@gobble\AM@pagelist}%
}
\newcommand{\AM@readlisti}{}
\def\AM@readlisti#1,{%
  \def\AM@temp{#1}%
  \ifx\END#1
  \else
    \AM@checkrange#1-\END
    \expandafter\AM@readlisti
  \fi
}
\newcommand{\AM@checkrange}{}
\def\AM@checkrange#1-#2\END{%
  \edef\AM@tempi{\AM@trim@space{#1}}%
  \ifx\\#2\\%
    \AM@checkinteger{\AM@tempi}%
    \ifAM@integer\AM@append{\AM@tempi}%
    \else
      \expandafter\ifx\expandafter\\\AM@tempi\\\AM@append{}%
      \else\AM@setnewdocname{\AM@tempi}\fi
    \fi
  \else
    \expandafter\ifx\expandafter\\\AM@tempi\\%
      \@tempcnta=1\relax
      \AM@checklast#2\END
    \else
      \AM@checkinteger{\AM@tempi}%
      \ifAM@integer
        \@tempcnta=\AM@tempi\relax
        \AM@checklast#2\END
      \else
        \AM@setnewdocname{\AM@temp}%
      \fi
    \fi
  \fi
}
\newcommand{\AM@checklast}{}
\def\AM@checklast#1-\END{%
  \edef\AM@tempii{\AM@trim@space{#1}}%
  \expandafter\ifx\expandafter\\\AM@tempii\\
    \pdfximage{\AM@currentdocname}%
    \@tempcntb=\the\pdflastximagepages\relax
    \advance\@tempcntb\@ne
    \whiledo{\@tempcnta<\@tempcntb}{%
      \AM@append{\the\@tempcnta}%
      \advance\@tempcnta\@ne
    }%
  \else
    \AM@checkinteger{\AM@tempii}%
    \ifAM@integer
      \@tempcntb=\AM@tempii\relax
      \advance\@tempcntb\@ne
      \whiledo{\@tempcnta<\@tempcntb}{%
        \AM@append{\the\@tempcnta}%
        \advance\@tempcnta\@ne
      }%
    \else
      \AM@setnewdocname{\AM@temp}%
    \fi
  \fi
}
\newcommand{\AM@setnewdocname}[1]{%
  \ifAM@defaultone
    \AM@append{1}%
  \fi
  \edef\AM@temp{\AM@trim@space{#1}}%
  \IfFileExists{\AM@temp}{\edef\AM@currentdocname{\AM@temp}}
    {\IfFileExists{\AM@temp.pdf}{\edef\AM@currentdocname{\AM@temp.pdf}}
       {\PackageError{pdfpages}{Cannot find file `\AM@temp'}{}}}%
  \AM@defaultonetrue
}
\newcommand{\AM@append}[1]{%
  \edef\AM@doclist{\AM@doclist,\AM@currentdocname}%
  \edef\AM@pagelist{\AM@pagelist,#1}%
  \ifAM@doublepages
    \edef\AM@doclist{\AM@doclist,\AM@currentdocname}%
    \edef\AM@pagelist{\AM@pagelist,#1}%
  \fi
  \AM@defaultonefalse
}
\newif\ifAM@endoflist\AM@endoflistfalse
\newcommand{\AM@getfirst}{}
\def\AM@getfirst#1{\expandafter\AM@getfirsti#1,\END#1\END}
\newcommand{\AM@getfirsti}{}
\def\AM@getfirsti#1,#2\END#3\END{%
  \edef#3{#2}%
  \ifx\\#2\\%
    \setboolean{AM@endoflist}{true}%
    \def#3{}%
  \else
    \edef#3{\AM@getfirstii#2\END}%
  \fi
  \toks@{#1}%
}
\newcommand{\AM@getfirstii}{}
\def\AM@getfirstii#1,\END{#1}
\newcommand{\AM@readfirst}{}
\newcommand{\AM@readfirsti}{}
\def\AM@readfirst#1{\expandafter\AM@readfirsti#1,\END}
\def\AM@readfirsti#1,#2\END{\toks@{#1}}
\newcommand{\AM@getlast}{}
\def\AM@getlast#1{%
  \let\AM@temp\relax
  \expandafter\AM@getlasti#1,\END
  \@ifundefined{AM@temp}{\def#1{}}{\edef#1{\AM@temp}}%
}
\newcommand{\AM@getlasti}{}
\def\AM@getlasti#1,#2\END{%
  \ifx\\#2\\%
    \def\AM@lastitem{#1}%
  \else
    \@ifundefined{AM@temp}
      {\edef\AM@temp{#1}}
      {\edef\AM@temp{\AM@temp,#1}}%
    \AM@getlasti#2\END
  \fi
}
\newcommand{\AM@getlastn}{}
\def\AM@getlastn#1#2{%
  \let\AM@templist\relax
  \@tempcnta=\z@
  \loop
  \ifnum\@tempcnta<#2
    \AM@getlast{#1}%
    \@ifundefined{AM@templist}
      {\edef\AM@templist{\AM@lastitem}}
      {\edef\AM@templist{\AM@lastitem,\AM@templist}}%
    \advance\@tempcnta\@ne
  \repeat
  \edef\AM@lastnitems{\AM@templist}%
}
\newif\ifAM@again\AM@againtrue
\newcommand{\AM@count}{}
\def\AM@count#1{%
  \edef\AM@templist{#1}%
  \loop
    \AM@getlast{\AM@templist}%
    \expandafter\ifx\expandafter\\\AM@lastitem\\%
    \else
      \AM@againfalse
      \expandafter\ifx\expandafter\\\AM@templist\\%
        \edef\AM@templist{\AM@lastitem}%
      \else
        \edef\AM@templist{\AM@templist,\AM@lastitem}%
      \fi
      \@tempcnta=\z@
      \expandafter\AM@counti\AM@templist,\END,
    \fi
  \ifAM@again
  \repeat
}
\newcommand{\AM@counti}{}
\def\AM@counti#1,{%
  \ifx\END#1
  \else
    \advance\@tempcnta\@ne
    \expandafter\AM@counti
  \fi
}
\newif\ifAM@resort@end\AM@resort@endfalse
\newcommand{\AM@resort}{}
\def\AM@resort{%
  \def\AM@resortedpagelist{}%
  \def\AM@resorteddoclist{}%
  \def\AM@xnupi{\@ne}%
  \def\AM@ynupi{\@ne}%
  \AM@count{\AM@lastnpages}%
  \def\AM@xnuplast{%
    \the\@tempcnta - (\the\@tempcnta / \AM@xnup * \AM@xnup) + 1}%
  \def\AM@ynuplast{1 + (\the\@tempcnta / \AM@xnup)}%
  \setlength{\@tempdima}{\p@*(\AM@xnuplast)}%
  \edef\AM@xnuplast{\strip@pt\@tempdima}%
  \setlength{\@tempdima}{\p@*(\AM@ynuplast)}%
  \edef\AM@ynuplast{\strip@pt\@tempdima}%
  \whiledo{\not\boolean{AM@resort@end}}{%
    \@tempcnta=\AM@ynupi\relax
    \@tempcntb=\AM@ynuplast\relax
    \ifnum\@tempcnta=\@tempcntb
        \@tempcnta=\AM@xnupi\relax
        \@tempcntb=\AM@xnuplast\relax
        \ifnum\@tempcnta<\@tempcntb
          \AM@getfirst{\AM@lastndocs}%
          \edef\AM@firstdocitem{\the\toks@}%
          \AM@getfirst{\AM@lastnpages}%
          \edef\AM@resortedpagelist{\AM@resortedpagelist,\the\toks@}%
          \edef\AM@resorteddoclist{%
            \AM@resorteddoclist,\AM@firstdocitem}%
        \else
          \edef\AM@resortedpagelist{\AM@resortedpagelist,}%
          \edef\AM@resorteddoclist{\AM@resorteddoclist,\AM@phantomdoc}%
        \fi
    \else
      \ifnum\@tempcnta<\@tempcntb
        \AM@getfirst{\AM@lastndocs}%
        \edef\AM@firstdocitem{\the\toks@}%
        \AM@getfirst{\AM@lastnpages}%
        \edef\AM@resortedpagelist{\AM@resortedpagelist,\the\toks@}%
        \edef\AM@resorteddoclist{\AM@resorteddoclist,\AM@firstdocitem}%
      \else
        \edef\AM@resortedpagelist{\AM@resortedpagelist,}%
        \edef\AM@resorteddoclist{\AM@resorteddoclist,\AM@phantomdoc}%
      \fi
    \fi
    \@tempcnta=\AM@ynupi\relax
    \advance\@tempcnta\@ne
    \edef\AM@ynupi{\the\@tempcnta}%
    \@tempcntb=\AM@ynup\relax
    \ifnum\@tempcnta>\@tempcntb
      \@tempcntb=\AM@xnupi\relax
      \advance\@tempcntb\@ne
      \edef\AM@xnupi{\the\@tempcntb}%
      \def\AM@ynupi{\@ne}%
      \@tempcnta=\AM@xnup\relax
      \ifnum\@tempcntb>\@tempcnta
        \setboolean{AM@resort@end}{true}%
      \fi
    \fi
  }%
  \edef\AM@resortedpagelist{\expandafter\@gobble\AM@resortedpagelist}%
  \edef\AM@resorteddoclist{\expandafter\@gobble\AM@resorteddoclist}%
}
\newif\ifAM@scale
\newcommand{\AM@remove@scale}{}
\def\AM@remove@scale#1{%
  \def\AM@options{}%
  \AM@remove@scalei#1,\END,
}
\newcommand{\AM@remove@scalei}{}
\def\AM@remove@scalei#1,{%
  \ifx\END#1
  \else
    \AM@scalefalse
    \AM@remove@scaleii#1=\END
    \ifAM@scale
    \else
      \ifx\empty\AM@options
        \edef\AM@options{#1}%
      \else
        \toks@\expandafter{\AM@options,#1}%
        \edef\AM@options{\the\toks@}%
      \fi
    \fi
    \expandafter\AM@remove@scalei
  \fi
}
\newcommand{\AM@remove@scaleii}{}
\def\AM@remove@scaleii#1=#2\END{%
  \ifx\\#2\\%
  \else
    \def\AM@temp{#1}%
    \edef\AM@temp{\AM@trim@space{\AM@temp}}%
    \ifthenelse{\equal{scale}{\AM@temp}}{\AM@scaletrue}{}%
  \fi
}
\newif\ifAM@pdfpages@options
\newif\ifAM@scale
\newcommand{\AM@split@options}{}
\def\AM@split@options#1#2{%
  \def\AM@param{#1}%
  \@temptokena{}%
  \AM@split@optionsi#2,\END,
}
\def\AM@split@optionsi#1,{%
  \ifx\END#1
  \else
    \AM@pdfpages@optionsfalse \AM@scalefalse
    \AM@split@optionsii#1=\END
    \ifthenelse{\equal{\AM@param}{pdfpages}}
      {\ifAM@pdfpages@options
          \@temptokena\expandafter{\the\@temptokena,#1}%
       \fi}{}%
    \ifthenelse{\equal{\AM@param}{Gin}}
      {\ifAM@pdfpages@options\else
         \@temptokena\expandafter{\the\@temptokena,#1}%
       \fi}{}%
    \ifthenelse{\equal{\AM@param}{Gin@noscale}}
      {\ifAM@pdfpages@options\else
         \ifAM@scale\else
           \@temptokena\expandafter{\the\@temptokena,#1}%
         \fi
       \fi}{}%
    \expandafter\AM@split@optionsi
  \fi
}
\newcommand{\AM@split@optionsii}{}
\def\AM@split@optionsii#1=#2\END{%
  \edef\AM@temp{\AM@trim@space{#1}}%
  \ifthenelse{\equal{pages}{\AM@temp}\or
              \equal{nup}{\AM@temp}\or
              \equal{deltax}{\AM@temp}\or
              \equal{deltay}{\AM@temp}\or
              \equal{delta}{\AM@temp}\or
              \equal{offset}{\AM@temp}\or
              \equal{frame}{\AM@temp}\or
              \equal{openright}{\AM@temp}\or
              \equal{pagecommand}{\AM@temp}\or
              \equal{landscape}{\AM@temp}\or
              \equal{turn}{\AM@temp}\or
              \equal{column}{\AM@temp}\or
              \equal{columnstrict}{\AM@temp}\or
              \equal{noautoscale}{\AM@temp}\or
              \equal{thread}{\AM@temp}\or
              \equal{threadname}{\AM@temp}\or
              \equal{link}{\AM@temp}\or
              \equal{linkfit}{\AM@temp}\or
              \equal{linkname}{\AM@temp}\or
              \equal{linktodoc}{\AM@temp}\or
              \equal{linktodocfit}{\AM@temp}\or
              \equal{linkfilename}{\AM@temp}\or
              \equal{fitpaper}{\AM@temp}\or
              \equal{addtotoc}{\AM@temp}\or
              \equal{addtolist}{\AM@temp}\or
              \equal{doublepages}{\AM@temp}\or
              \equal{signature}{\AM@temp}}{\AM@pdfpages@optionstrue}{}%
  \ifthenelse{\equal{scale}{\AM@temp}}{\AM@scaletrue}{}%
}
\newcommand{\AM@trim@space}{}\newcommand{\AM@trim@spacei}{}
\newcommand{\AM@trim@spaceii}{}
\def\AM@trim@space#1{%
  \expandafter\AM@trim@spacei\expandafter{\ifdim\z@=0pt#1}\fi}
\def\AM@trim@spacei#1{\AM@trim@spaceii#1 \END}
\def\AM@trim@spaceii#1 #2\END{#1}
\def\AM@trim@leadingspace#1{\ifdim\z@=0pt#1\fi}
\newif\ifAM@phantompage
\newcommand*{\AM@isphantom}{%
  \expandafter\ifx\expandafter\\\AM@page\\%
    \let\AM@page\AM@phantompage
    \let\AM@ph\phantom
    \AM@phantompagetrue
  \else
    \let\AM@ph\relax
    \AM@phantompagefalse
  \fi
}
\newcommand{\AM@hyper}{%
  \ifAM@link
    \pdfdest name {\AM@linkname.\AM@page} \AM@linkfit%
  \fi
  \ifAM@linktodoc
    \pdfannot width \wd\@tempboxa
              height \ht\@tempboxa
              depth \dp\@tempboxa
              {/Subtype /Link /Border [0 0 0]
               /A << /S /GoToR
                     /F (\AM@linkfilename)
                     /D [\AM@page@linktodoc \AM@linktodocfit]
                     \ifAM@newwindow/NewWindow true\fi >>}%
  \fi
  \ifAM@thread
      \pdfthread width \wd\@tempboxa
                 height \ht\@tempboxa
                 depth \dp\@tempboxa
                 attr {\threadinfodict}%
                 name {\AM@threadname}%
  \fi
}
\newcommand{\AM@openright}{}
\def\AM@openright{%
  \edef\AM@pagelist{,\AM@pagelist}%
  \edef\AM@doclist{\AM@phantomdoc,\AM@doclist}%
}
\newcommand{\AM@countpagelist}{}
\def\AM@countpagelist{%
  \@tempcnta=\z@
  \expandafter\AM@countpagelisti\AM@pagelist,\END,
}
\newcommand{\AM@countpagelisti}{}
\def\AM@countpagelisti#1,{%
  \ifx\END#1
  \else
    \advance\@tempcnta\@ne
    \expandafter\AM@countpagelisti
  \fi
}
\newcommand{\AM@filluppagelist}{}
\def\AM@filluppagelist{%
  \@tempcnta=\AM@xnup\relax
  \@tempcntb=\AM@ynup\relax
  \multiply\@tempcnta\@tempcntb
  \edef\AM@nup{\the\@tempcnta}%
  \AM@countpagelist
  \@tempcntb=\@tempcnta
  \divide\@tempcntb\AM@nup
  \multiply\@tempcntb\AM@nup
  \advance\@tempcnta-\@tempcntb
  \ifnum\@tempcnta=\z@
    \else
      \advance\@tempcnta-\AM@nup
      \multiply\@tempcnta\m@ne
  \fi
  \whiledo{\@tempcnta > \z@}{%
    \let\saveAM@pagelist\AM@pagelist
    \edef\AM@pagelist{\saveAM@pagelist,}%
    \advance\@tempcnta\m@ne
    \let\saveAM@doclist\AM@doclist
    \edef\AM@doclist{\saveAM@doclist,\AM@phantomdoc}%
  }%
}
\newcommand{\AM@prepare@signature}{}
\def\AM@prepare@signature{%
  \def\AM@newpagelist{}%
  \def\AM@newdoclist{}%
  \@tempcnta=\AM@signature\relax
  \divide\@tempcnta by 4
  \multiply\@tempcnta by 4
  \ifnum\@tempcnta=0\@tempcnta=4\fi
  \edef\AM@signature{\the\@tempcnta}%
  \AM@countpagelist
  \count@=\@tempcnta
  \@tempcntb=\AM@signature\relax
  \divide\count@\@tempcntb
  \multiply\count@\@tempcntb
  \advance\@tempcnta-\count@
  \ifnum\@tempcnta=0 \@tempcntb=0
  \else\advance\@tempcntb-\@tempcnta
  \fi
  \whiledo{\@tempcntb>\z@}{%
    \edef\AM@pagelist{\AM@pagelist,}%
    \edef\AM@doclist{\AM@doclist,\AM@phantomdoc}%
    \advance\@tempcntb\m@ne
  }%
  \def\AM@sort{%
    \def\AM@sigpagelist{}%
    \def\AM@sigdoclist{}%
    \@tempcntb=\AM@signature\relax
    \AM@getlastn{\AM@pagelist}{\@tempcntb}%
    \edef\AM@lastnpages{\AM@lastnitems}%
    \AM@getlastn{\AM@doclist}{\@tempcntb}%
    \edef\AM@lastndocs{\AM@lastnitems}%
    \@tempcnta=0
    \def\AM@first{%
      \AM@getfirst{\AM@lastnpages}%
      \edef\AM@sigpagelist{\AM@sigpagelist,\the\toks@}%
      \AM@getfirst{\AM@lastndocs}%
      \edef\AM@sigdoclist{\AM@sigdoclist,\the\toks@}%
    }%
    \def\AM@last{%
      \AM@getlast{\AM@lastnpages}%
      \edef\AM@sigpagelist{\AM@sigpagelist,\AM@lastitem}%
      \AM@getlast{\AM@lastndocs}%
      \edef\AM@sigdoclist{\AM@sigdoclist,\AM@lastitem}%
    }%
    \whiledo{\@tempcnta<\@tempcntb}{%
      \ifAM@landscape
        \AM@last\AM@first\AM@last\AM@first
      \else
        \AM@first\AM@last\AM@first\AM@last
      \fi
      \advance\@tempcnta by 4
    }%
    \edef\AM@newpagelist{\AM@sigpagelist\AM@newpagelist}%
    \edef\AM@newdoclist{\AM@sigdoclist\AM@newdoclist}%
    \ifx\AM@pagelist\@empty
    \else\expandafter\AM@sort
    \fi
  }%
  \AM@sort
  \edef\AM@pagelist{\expandafter\@gobble\AM@newpagelist}%
  \edef\AM@doclist{\expandafter\@gobble\AM@newdoclist}%
  \ifdim\pdfpagewidth<\pdfpageheight
    \def\AM@xnup{\@ne}\def\AM@ynup{\tw@}%
  \else
    \def\AM@xnup{\tw@}\def\AM@ynup{\@ne}%
  \fi
}
\newcommand*{\AM@setphantom}{%
  \expandafter\AM@setphantompage\AM@pagelist,\END,
  \expandafter\AM@setphantomdoc\AM@doclist,\END
}
\newcommand{\AM@setphantompage}{}
\def\AM@setphantompage#1,{%
  \def\AM@gobble##1\END,{}%
  \ifx\\#1\\%
    \expandafter\AM@setphantompage
  \else
    \def\AM@phantompage{#1}%
    \expandafter\AM@gobble
  \fi
}
\newcommand{\AM@setphatomdoc}{}
\def\AM@setphantomdoc#1,#2\END{\edef\AM@phantomdoc{#1}}
\newcommand{\AM@addtotoc@hook}{\relax}
\newcommand{\AM@addtotoc}{}
\def\AM@addtotoc{%
  \begingroup
  \def\@seccntformat##1{}\def\@makechapterhead##1{}%
  \def\@endpart{}\def\partname{}%
  \def\autodot{}% KOMA classes
  \let\AM@addcontentsline\addcontentsline
  \def\addcontentsline##1##2##3{%
    \AM@addcontentsline{##1}{##2}{##3}%
    \def\thepart{}}%
  \AM@addtotoc@hook
  \edef\AM@temp{{\AM@toc@section}{\AM@toc@level}%
           {\z@}{\z@}{\z@}{}[\AM@trim@leadingspace\AM@toc@heading]{}}%
  \edef\AM@tempi{\noexpand\csname @\AM@toc@section\noexpand\endcsname%
                 [\AM@trim@leadingspace\AM@toc@heading]{}}%
  \@ifundefined{@\AM@toc@section}
    {\expandafter\@sect\AM@temp
     \hskip\z@\par\vskip-\parskip\vskip-\baselineskip\hskip\z@}
    {\AM@tempi}%
  \label{\AM@toc@label}%
  \endgroup
}
\newcommand{\AM@parse@toclist}{}
\def\AM@parse@toclist{%
  \ifx\AM@toclist\empty \def\AM@toc@page{0}%
  \else \expandafter\AM@parse@toclisti\AM@toclist\END
  \fi
}
\newcommand{\AM@parse@toclisti}{}
\def\AM@parse@toclisti#1,#2,#3,#4,#5,#6\END{%
  \def\AM@toc@page{\AM@trim@space{#1}}%
  \def\AM@toc@section{\AM@trim@space{#2}}%
  \def\AM@toc@level{\AM@trim@space{#3}}%
  \def\AM@toc@heading{#4}%
  \def\AM@toc@label{\AM@trim@space{#5}}%
  \AM@checkinteger{\AM@toc@page}%
  \ifAM@integer\else
    \PackageError{pdfpages}
         {Missing number.\MessageBreak
          Page number in option `addtotoc' is not a number}
         {See the pdfpages manual for explanation.}%
   \fi
}
\newcommand{\AM@rm@from@toclist}{}
\def\AM@rm@from@toclist{%
    \expandafter\AM@rm@from@toclisti\AM@toclist\END
}
\newcommand{\AM@rm@from@toclisti}{}
\def\AM@rm@from@toclisti#1,#2,#3,#4,#5,#6\END{%
  \def\AM@toclist{#6}%
}
\newcommand{\AM@addtolist@hook}{\relax}
\newcommand{\AM@addtolist}{}
\def\AM@addtolist{
  \def\@captype{\AM@lof@list}%
  \long\def\@makecaption##1##2{}%
  \let\@fs@capt\relax% float.sty
  \caption{\AM@lof@heading}%
  \AM@addtolist@hook
  \@ifundefined{hyper@@anchor}{}{%
    \@ifundefined{float@caption}{%
      \hyper@@anchor{\@currentHref}{\relax}%
  }{}}%
  \label{\AM@lof@label}%
  \vskip-\baselineskip
}
\newcommand{\AM@parse@loflist}{}
\def\AM@parse@loflist{%
  \ifx\AM@loflist\empty \def\AM@lof@page{0}%
  \else \expandafter\AM@parse@loflisti\AM@loflist\END
  \fi
}
\newcommand{\AM@parse@loflisti}{}
\def\AM@parse@loflisti#1,#2,#3,#4,#5\END{%
  \def\AM@lof@page{\AM@trim@space{#1}}%
  \def\AM@lof@list{\AM@trim@space{#2}}%
  \def\AM@lof@heading{#3}%
  \def\AM@lof@label{\AM@trim@space{#4}}%
  \AM@checkinteger{\AM@lof@page}%
  \ifAM@integer\else
    \PackageError{pdfpages}
         {Missing number.\MessageBreak
          Page number in option `addtolist' is not a number}
         {See the pdfpages manual for explanation.}%
  \fi
}
\newcommand{\AM@rm@fromloflist}{}
\def\AM@rm@from@loflist{%
    \expandafter\AM@rm@from@loflisti\AM@loflist\END
}
\newcommand{\AM@rm@from@loflisti}{}
\def\AM@rm@from@loflisti#1,#2,#3,#4,#5\END{%
  \def\AM@loflist{#5}%
}
\newcommand{\AM@toclof}{}
\def\AM@toclof#1{%
  \AM@parse@toclist
  \whiledo{#1=\AM@toc@page}{%
    \ifx\AM@toclist\empty
    \else
      \AM@addtotoc
      \AM@rm@from@toclist
      \def\AM@toc@page{0}%
      \AM@parse@toclist
    \fi
  }%
  \AM@parse@loflist
  \whiledo{#1=\AM@lof@page}{%
    \ifx\AM@loflist\empty
    \else
      \AM@addtolist
      \AM@rm@from@loflist
      \def\AM@lof@page{0}%
      \AM@parse@loflist
    \fi
  }%
}
\define@key{pdfpages}{pages}{\def\AM@pagestemp{#1}}
\define@key{pdfpages}{nup}{\AM@parse@nup#1x\END}
\define@key{pdfpages}{deltax}{\AM@parse@deltax#1 \\}
\define@key{pdfpages}{deltay}{\AM@parse@deltay#1 \\}
\define@key{pdfpages}{delta}{\AM@parse@delta#1 \\}
\define@key{pdfpages}{offset}{\AM@parse@offset#1 \\}
\define@key{pdfpages}{frame}[true]{\setboolean{AM@frame}{#1}}
\define@key{pdfpages}{openright}[true]{\setboolean{AM@openright}{#1}}
\define@key{pdfpages}{pagecommand}{\def\AM@pagecommand{#1}}
\define@key{pdfpages}{landscape}[true]{\setboolean{AM@landscape}{#1}}
\define@key{pdfpages}{turn}[true]{\setboolean{AM@turn}{#1}}
\define@key{pdfpages}{column}[true]{\setboolean{AM@column}{#1}}
\define@key{pdfpages}{columnstrict}[true]%
                     {\setboolean{AM@columnstrict}{#1}}
\define@key{pdfpages}{noautoscale}[true]%
                     {\setboolean{AM@noautoscale}{#1}}
\define@key{pdfpages}{thread}[true]{\setboolean{AM@thread}{#1}}
\define@key{pdfpages}{threadname}{\def\AM@threadname{#1}}
\define@key{pdfpages}{link}[true]{\setboolean{AM@link}{#1}}
\define@key{pdfpages}{linkfit}{\def\AM@linkfit{#1}}
\define@key{pdfpages}{linkname}{\def\AM@linkname@option{#1}}
\define@key{pdfpages}{linktodoc}[true]{\setboolean{AM@linktodoc}{#1}}
\define@key{pdfpages}{linktodocfit}{\def\AM@linktodocfit{#1}}
\define@key{pdfpages}{linkfilename}{\pdfstringdef\AM@linkfilename{#1}%
                               \AM@linkfilenametrue}
\define@key{pdfpages}{fitpaper}[true]{\setboolean{AM@fitpaper}{#1}}
\define@key{pdfpages}{addtotoc}{\def\AM@toclist{#1,}}
\define@key{pdfpages}{addtolist}{\def\AM@loflist{#1,}}
\define@key{pdfpages}{doublepages}[true]%
                     {\setboolean{AM@doublepages}{#1}}
\define@key{pdfpages}{signature}{\def\AM@signature{#1}}
\newcommand{\AM@parse@nup}{}
\def\AM@parse@nup#1x#2\END{%
  \ifx\\#2\\%
    \def\AM@shortnupsyntax{}%
    \def\AM@xnup{\@ne}%
    \def\AM@ynup{\@ne}%
    \ifnum#1=\tw@
      \def\AM@xnup{\tw@}%
      \def\AM@ynup{\@ne}%
    \fi
    \ifnum#1=4
      \def\AM@xnup{\tw@}%
      \def\AM@ynup{\tw@}%
    \fi
  \else
    \def\AM@xnup{#1}%
    \AM@parse@nupi#2%
  \fi
}
\def\AM@parse@nupi#1x{\def\AM@ynup{#1}}
\def\AM@parse@deltax#1 #2\\{\AMGin@defaultbp\AM@deltax{#1}}
\def\AM@parse@deltay#1 #2\\{\AMGin@defaultbp\AM@deltay{#1}}
\def\AM@parse@delta#1 #2 #3\\{%
  \AMGin@defaultbp\AM@deltax{#1}%
  \AMGin@defaultbp\AM@deltay{#2}}
\def\AM@parse@offset#1 #2 #3\\{%
  \AMGin@defaultbp\AM@xoffset{#1}%
  \AMGin@defaultbp\AM@yoffset{#2}}
\def\AMGin@defaultbp#1#2{%
  \afterassignment\AMGin@def@bp\dimen@#2bp\relax{#1}{#2}}
\def\AMGin@def@bp#1\relax#2#3{%
   \if!#1!%
     \def#2{#3bp}%
    \else
      \dimen@.99626\dimen@
      \edef#2{\strip@pt\dimen@ bp}%
    \fi
}
\InputIfFileExists{pdfpages.fix}{%
  \PackageInfo{pdfpages}{Loading patch file `pdfpages.fix'}}{}
\endinput
%%
%% End of file `pdfpages.sty'.


==> pf-section-2.tex <==
\section{Proofs from Section 2}

\subsection{Proof of Claim \ref{setlevelTime}} \label{setlevelApp}
%\begin{proof}
First, recall that the authentication process takes $O(\log^2 n)$ time.  %, as it is superseded by the runtime bound.

By Observation \ref{basicscan}, any non-active neighbor of $v$ scanned by the procedure  has level at most $\tilde \ell$.
We may restrict our attention to $v$'s neighbors of level at most $\tilde \ell$, since any time spent by the procedure
for handling active neighbors of $v$ of higher level is encapsulated within the authentication process.
%all non-active outgoing neighbors of $v$ at the beginning of the procedure's execution have level at most $\ell_v$.
%or in other words,  each neighbor of $v$ scanned by Procedure $\setlvl(v,\ell)$ is either active or has level at most $\tilde \ell$.
%For each of the at most $O(\log n)$ active outgoing neighbors $w$ of $v$ at the beginning of the procedure's execution, the procedure also spends $O(\log n)$ time
%for updating the relevant data structures and $\phi_v$ values.
Note that only $O(\log n)$ neighbors  of $v$ at the beginning of the procedure's execution may be active.
For each neighbor $w$ of $v$ of level at most $\tilde \ell$ (active or not),
the procedure spends at most $O(1)$ time for updating the appropriate data structures $\cO_v,\cI_v,\cO_w,\cI_w$,
and at most $O(\log n)$ time for updating the relevant $\phi_w$ values.  % in at most $|\ell - \ell_v|$ levels.
This, however, does not imply that the procedure's runtime is  $O((\phi_v(\tilde \ell + 1) + \log n)\cdot \log n)$,
as the set of neighbors of $v$ is not static,
%In fact, this runtime bound is not well-defined, as $\phi_v(\max\{\ell,\ell_v\})$ dynamically changes throughout the execution of this procedure.
 but rather changes dynamically throughout the procedure's execution.
In particular, the corresponding set $N_v(\tilde \ell+1)$ (of $v$'s neighbors of level lower than $\tilde \ell+1$) is not static.
%Therefore, the total time that the procedure takes for handling all relevant neighbors of $v$ at the beginning of the execution is
%bounded by $O((\phi_v(\tilde \ell + 1) + \log n)\cdot \log n)$,

% vertices of $N_v(\tilde \ell)$, i.e.,

%To prove the claim, one may show that only few vertices may  join $N_v(\tilde \ell)$.  % throughout this execution.
%There is no need for that, however.
A vertex $w$ joins $N_v(\tilde \ell+1)$ in one of two ways, the first is due to adversarial edge insertions.
%The remaining vertices that may join $N_v(\tilde \ell)$ are due to new edges added to the graph.
%Although we can bound the number of such vertices by $\phi_v(\tilde \ell)$, there is no need for that.
Whenever an edge $(v,w)$ adjacent to $v$ is added to the graph, the data structures are updated in $O(\log n)$ time.
This update of the data structures is not part of Procedure $\setlvl(v,\ell)$, but rather part of the procedure that handles the insertion of edge $(v,w)$,
namely Procedure $\ins$,  described in Section 2.5.

%Since the number of such vertices is at most $O(\log n)$, this authentication cost is at most $O(\log^2 n)$.

The second way for a vertex $w$ to join $N_v(\tilde \ell+1)$ is by
%First, we argue that at most $O(\log n)$ vertices join $N_v(\tilde \ell)$ due to level change.
%Note that any vertex joining $N_v(\tilde \ell)$ is
falling from level higher than $\tilde \ell$ to level at most $\tilde \ell$.
It is possible that $w$ changes its level throughout the execution of this procedure multiple times.
%The argument used for the case where $w$ is a new neighbor of $v$ remains valid here.
For every such change in level except for maybe the last, the data structures of $v$ are updated as part of the respective calls to Procedure $\setlvl(w,\cdot)$,
and more concretely, each time $w$ is removed from the $Active$ list throughout the execution of Procedure $\setlvl(v,\ell)$, the data structures of $v$ are updated accordingly.
Those data structures may be outdated only if $w$ belongs to the $Active$ list at the end of the execution of Procedure $\setlvl(v,\ell)$.
For this reason we scan the entire $Active$ list at that stage, spending $O(\log n)$ time per active neighbor of $v$ for updating the relevant data structures.
This update of the data structures is part of the authentication process, whose cost was already taken into account.

When a vertex $w$ leaves $N_v(\tilde \ell+1)$, the data structures of $v$ (either the old or the temporary ones) are updated accordingly.
As with vertices that join $N_v(\tilde \ell+1)$, this update of the data structures is not part of Procedure  $\setlvl(v,\ell)$.
If $w$ leaves $N_v(\tilde \ell+1)$ due to an edge deletion, this update is part of the procedure that handles the deletion of edge $(v,w)$,
namely Procedure $\del$,  described in Section 2.5.
The second way for a vertex $w$ to leave $N_v(\tilde \ell+1)$ is by
%First, we argue that at most $O(\log n)$ vertices join $N_v(\tilde \ell)$ due to level change.
%Note that any vertex joining $N_v(\tilde \ell)$ is
rising from level at most $\tilde \ell$ to level higher than $\tilde \ell$,
in which case the data structures of $v$ are updated either as part of the respective calls to Procedure $\setlvl(w,\cdot)$
or as part of the authentication process.
%Consequently, there is no extra cost due to vertices that leave $N_v(\tilde \ell+1)$.

When a vertex $w$ joins or leaves $N_v(\tilde \ell+1)$, the temporary data structures of $v$, namely $\cO'_v$ or  $\cI'_v$, are updated accordingly;
if $w$ joins $N_v(\tilde \ell+1)$,   these data structures are updated according to the new level of $w$.
Also, the data structures of each such neighbor are updated according to the destination level $\ell$ of $v$.
Hence there is no need for Procedure $\setlvl(v,\ell)$ to update the temporary data structures of $v$ nor to update the respective data structures of vertices
belonging to the temporary data structures of $v$, and the only cost due to vertices that join or leave $N_v(\tilde \ell+1)$ incurred by this procedure is that of merging the old data structures of $v$ with the new ones.
Merging $\cO_v$ with $\cO'_v$ takes constant time, and merging $\cI_v$ with $\cI'_v$ takes $O(\log n)$ time,
as we need to merge the respective lists $\cI_v[j]$ and $\cI'_v[j]$ one by one, possibly for each level $j \le \tilde \ell$.
Thus the extra cost due to vertices that join or leave $N_v(\tilde \ell+1)$ is $O(\log n)$.


%By Observation \ref{ob:basic}, any such vertex is handled by an execution thread of level at least $\tilde \ell$.
%Hence, by Lemma \ref{ob:time}, at most $O(\log^2 n)$ falling vertices will join $N_v(\tilde \ell)$
%throughout the execution of Procedure $\setlvl(v,\ell)$.
\ignore{
 which requires at least the same amount
of time as that required by the level-$\tilde \ell$ thread that executes Procedure $\setlvl(v,\ell)$.
The number of different threads running at any point in time is bounded by $O(\log n)$,
at most a single thread for each sub-scheduler at each of the $\log_\gamma (n-1)$ levels. (Recall that there are three different sub-schedulers at each level.)
Since each thread
Consequently,
}

%We have shown that the total runtime of the procedure spent for h$N_v(\tilde \ell)$
Summarizing, we have shown that $L_{\tilde \ell}(v) = O((\phi_v(\tilde \ell+1) + \log n) \cdot \log n)$.
\QED
%\end{proof}

\subsection{Zooming in on Procedure $\evalf$} \label{zoom}
%\vspace{7pt}
%\\
%\noindent
%{\bf Zooming in.~}
Recall that none of the values $\phi_v(\ell)$ and vertex sets $N_v(\ell)$, for $0 \le \ell \le \ell_v$, is maintained by the update algorithm,
and computing them is a process that is simulated over multiple update operations.
By the time we finish this process, some of the scanned neighbors of $v$ may have different levels than those they had at the time they were scanned.
Also, $v$ may acquire new neighbors at levels at most $\ell$ and lose others.
(Recall that we had similar problems with Procedure $\setlvl$.)
By Invariant \ref{1d}, when the execution of this procedure starts (i.e., just after $v$ becomes temporarily free),
every non-active neighbor of $v$ at level lower than $\ell_v$ is an outgoing neighbor of $v$.
We thus restrict our attention to the outgoing neighbors of $v$ in order to compute ``estimations'' for the values $\phi_v(j)$ and vertex sets $N_v(j)$,
for all $j \le \ell_v$. Once we finish computing these estimations, which might be simulated over multiple update operations,
we make these estimations accurate by running the authentication process described in Section 2.3.
Recall that the authentication process also considers vertices that belong to the $Active$ list at that stage.
%, and to resolve it we ran the authentication process .
It enables us to update the values $\phi_v(j)$ and vertex sets $N_v(j)$ in $O(\log^2 n)$ time, for $j \le \ell_v$,
and so this update can be carried out within time reserved for a single update operation, namely, either $\Delta$ or $\Delta'$ depending on the
thread executing the procedure, during which the $Active$ list remains intact. We then compute in $O(\log n)$ time the
the highest level $\ell, 0 \le \ell \le \ell_v$, where $\phi_v(\ell) \ge \gamma^{\ell}$, as well as the vertex set $N'_v(\ell)$.
\ignore{
A special attention should be given to vertices that belong to the $Active$ list during the authentication process.
For every such vertex that is falling or rising between levels $\ell'$ and $\ell''$, when updating the $\phi_v(\cdot)$ values and $N_v(\cdot)$ vertex sets,
its level is viewed as $\max\{\ell',\ell''\}$, i.e., the higher level among the two.
This stands in contrast to what we did in Procedure $\setlvl$,
where we viewed the level of a vertex that is falling or rising as its destination level. So the two procedures behave the same for rising vertices,
but behave differently for falling vertices. %This does not cause any inconsistencies, because whenever the vertex finishes the rising process, it
The reason we view a falling vertex as being in its old level is because we do not want vertices at intermediate levels to choose it
as their random mate. Such vertices are being handled by execution threads at lower levels than the one that handles the falling vertex,
and they may have to wait too much time for the vertex to complete its falling.
Note, however, that this is just a temporary inconsistency, which ends whenever the vertex finishes falling.
By being aware of this type of temporary inconsistencies, we can make sure to detect and resolve them on the fly.
}
%[[S: ignore --Once $v$ becomes temporarily free, it is added to that list.
%As a result, whenever any vertex is added or removed to and from this list, $v$ is updated about the new level of that vertex.]]
%Note that the list of outgoing neighbors change dynamically.
Following similar lines to those in the proof of Claim \ref{setlevelTime},
the runtime of this  process
%computing the values $\phi_v(\ell)$ and vertex sets $N_v(\ell)$, for $0 \le \ell \le \ell_v$,
is  $O(\phi_v(\ell_v+1) + O(\log n)) \cdot O(\log n)$,
where $\phi_v(\ell_v+1)$ denotes the number of $v$'s neighbors of level lower than $\ell_v + 1$ at the beginning  of the execution of this procedure.
By Invariant \ref{risei}, at any   time $\phi_v(\ell_v+1) = \gamma^{\ell_v+1} \cdot O(\log^2 n) = \gamma^{\ell_v} \cdot O(\log^3 n) $,
hence the runtime of this process is at most $O(\gamma^{\ell_v} \cdot \log^4 n)$.

For every vertex $w$ that joins or leaves $N_v(j)$ throughout the procedure's execution, for $j \le \ell_v + 1$, we make sure to update the
values $\phi_v(j)$ and vertex sets $N_v(j)$ accordingly, but this update is done as part of the respective call to Procedure $\setlvl(w,\cdot)$,
and is not part of Procedure $\evalf(v)$.
%just $O(\log n)$ falling vertices will join it and the number of vertices joining it due to new edges added to the graph is also small.
%we are able to compute the level $\ell$ as above and the corresponding vertex set $N_{\ell}(v)$ via a sequential scanning process that is simulated over multiple update operations.

Note that setting the level of $v$ to $\ell$ by calling $\setlvl(v,\ell)$ is another long process, which involves updating the relevant data structures.
During this process, the vertex set $N'_v(\ell)$ that we just computed may change. 
%Moreover, the values $\phi_v(j)$ that we computed may change too, for $\ell \le j \le \ell_v$.
%We next address these two issues.
%
%
%In particular, vertices from $N_v(\ell)$
For this reason, before initiating this process,
%we temporarily set the value of $\ell_v$ to $\ell$, and update the $Exceptions$ list about this change.
%These updates are carried out immediately, more accurately, within $O(\log n)$ time that is carried out before the next update operation.
we randomly sample a vertex $w$ from $N'_\ell(v)$ as the new mate of $v$.
As mentioned, we sample from at least $(1-\eps) \gamma^{\ell}$ vertices. 
(If we were to make the random sampling after the execution of the call to $\setlvl(v,\ell)$ is finished,
the sample space could a-priori be much smaller than  $(1-\eps) \gamma^{\ell}$, which would, in turn, invalidate our almost-maximality guarantee.
Although it is not difficult to prove that the sample space does not reduce significantly during the call to $\setlvl(v,\ell)$, we prefer to avoid such a proof.)
%For technical reasons, if $|N'_{\ell}(v)| > \gamma^{\ell}$, we sample from precisely $\gamma^{\ell}$ vertices of $N'_{\ell}(v)$.)
Note that $w$ is not active at this moment, and in particular, is not in the process of falling or rising;
we then add $w$  to the $Active$ list.
It is crucial that the new mate $w$ of $v$ will be at level at most $\ell-1$.  % and that it is chosen uniformly at random from $2^{\ell}$ options.
 %but we made sure that both the source and destination levels of $w$ are bounded by $\ell-1$.
%Consequently, the execution thread handling $w$ is of level bounded by $\ell-1$, which is lower than the level of the execution thread handling $v$.
%In this case, there are several cases as to how to proceed;
%one of them is that the execution thread of $v$ would just wait for $w$ to finish falling or rising, and only then take control on it and proceed.
%Another option is to re-sample another random mate. If all these attempts reach active vertices, this means that the number of neighbors at lower level is logarithmic,
%and we can handle the vertex deterministically. (For more details, see Appendix \ref{exceptions}.)
%Regardless of this fact, however,
We argue that the random sampling of $w$ can be carried out within the time $\Delta$ or $\Delta'$ reserved for a single update operation.
(If we were to randomly sample $w$ via a   procedure whose runtime is linear in the sample space, then we would need to prove that the sample space does not reduce significantly during
the execution of this procedure, and we prefer to avoid such a proof.)  % Although it is not difficult to prove this, there is no need for it.)
To this end, the set $N'_\ell(v)$  that we just computed should be stored via a data structure that allows for fast retrieval of a random element,
such as a balanced (of logarithmic depth) tree in which every node is associated with a vertex of $N'_\ell(v)$ via mutual pointers, 
and it also holds a counter for the number of nodes in its subtree.
%Observe that the tree is constructed 
This tree has to be maintained in the time interval required for constructing it, during which some elements may leave the tree while others may join it.
In particular, any vertex leaving/joining $N'_\ell(v)$ throughout this time interval triggers a node insertion/removal to/from the tree, which requires $O(\log n)$ time.  % whereas updating a simple linked list takes constant time, as we did  that .
%whereas inserting/deleting an element to/from a doubly-linked list takes constant time.
Note, however, that the time needed by our algorithm to update the various $\phi_v$ counters
%and the update time per element joining/leaving the data structure was upper bounded by $O(\log n)$ and not constant,
%particularly due to vertices falling and rising) 
following %the time needed to update the relevant $\phi$ values per 
a fall/rise of a single neighbor of $v$ is also logarithmic, hence the overhead due to maintaining this tree is negligible.
%More concretely, we can store the set of non-active neighbors of $v$ with level precisely $j$, for $j \le \ell_v$, via such a tree $T_j(v)$ of pointers to those neighbors (with %mutual pointers),
%then the set $N'_v(\ell)$ is obtained as the union of the vertices pointed to by elements in the arrays $A_0(v),A_1(v),\ldots,A_{\ell-1}(v)$; for efficiency reasons, we do not %include in this union more than $\gamma^{\ell}$ elements.
%Since there are only $O(\log n)$ such arrays, 
Since the depth of this  tree is $O(\log n)$, it is straightforward to retrieve a random vertex from $N'_v(\ell)$ in $O(\log n)$ time, 
and we can easily make sure not to sample from more than $\gamma^{\ell}$ options.
%(In fact, even if we perform the random sampling within time that is linear in the size of $N_v(\ell)$,
%this sampling step can be simulated within $O(|N_v(\ell)|/\Delta)$ update operations, and it can be shown that during this time interval only few vertices may leave $N_\ell(v)$.)

Note also that during the call to  $\setlvl(v,\ell)$, the values $\phi_v(j)$ that we computed may change, for $\ell+1 \le j \le \ell_v$.
Recall that the level of $v$ during this falling of $v$ is viewed as its destination level $\ell$. At the beginning of this falling
(i.e., when the execution of the call to $\setlvl(v,\ell)$ starts) we have $\phi_v(j) < \gamma^{j}$, for all $\ell + 1 \le j \le \ell_v$.
These $\phi_v(j)$ values may grow during this falling, possibly beyond the threshold $\gamma^j \cdot O(\log^2 n)$ required by Invariant \ref{risei}.
In this case some sub-schedulers of $\rise$ may need to raise $v$ while $v$ is falling, which triggers a conflict between those sub-schedulers and the sub-scheduler executing the call to $\setlvl(v,\ell)$. We address this issue in App.\ \ref{mainc}.



Next, the same thread continues to setting the levels of $v$ and $w$ to $\ell$,
by executing Procedure $\setlvl(v,\ell)$ and then executing Procedure $\setlvl(w,\ell)$.
By Claim \ref{setlevelTime}, the runtime of these calls is bounded by $L_{\ell_v}(v) =  O((\phi_v(\ell_v+1) + \log n) \cdot \log n)$
and $L_{\ell}(w) =  O((\phi_w(\ell+1) + \log n) \cdot \log n)$, where $\phi_v(\ell_v+1)$ (respectively, $\phi_w(\ell+1)$)
stands for the number of neighbors of $v$ (resp., $w$) of level lower than $\ell_v+1$ (resp., $\ell+1$) just before the call to $\setlvl(v,\ell)$
%and stands for the number of neighbors of $w$ of level lower than $\ell$ just before the call to
(resp., $\setlvl(w,\ell)$).
By Invariant \ref{risei}, $\phi_v(\ell_v+1) = \gamma^{\ell_v+1} \cdot O(\log^2 n)$ and $\phi_w(\ell+1) = \gamma^{\ell+1} \cdot O(\log^2 n)
= \gamma^{\ell} \cdot O(\log^3 n)$,
hence the runtime of these calls   is $O(\gamma^{\ell_v} \cdot \log^4 n)$.
We then match $v$ with $w$, thus creating a new level-$\ell$ matched edge.

Finally, assuming $w$ was previously matched to $w'$, the vertex $w'$ becomes temporarily free.
By Invariant \ref{first}(b), the level of $w'$ is the same as the level of $w$ before executing Procedure $\setlvl(w,\ell)$,
hence it is at most $\ell-1$. We use the same thread to handle $w'$ recursively by calling $\evalf(w')$.
%we can scan list of outgoing neighbors of $v$, as well as the $Exceptions$ list, in the naive way.
%Although this process is simulated over multiple update operations, we are guaranteed to end up with an accurate state of affairs.
%At that time $v$ scans the entire $Exceptions$ list and verifies the updated level of vertices in that list.

Note that if the original level $\ell_v$ of $v$ is 0, then $\phi_v(0) \le \phi_v(1) = O(\log^3 n)$ by Invariant \ref{risei}.
Computing $\phi_v(0)$ and $N_v(0)$, including the authentication process, takes $O(\phi_v(1) + O(\log n)) \cdot O(\log n) = O(\log^4 n)$ time.
If $\phi_v(0) = 0$, then $v$ remains free, and the runtime of the call to $\setlvl(v,-1)$ is
$O(\phi_v(0) + O(\log n)) \cdot O(\log n) = O(\log^2 n)$ by Claim \ref{setlevelTime}.
Otherwise $\phi_v(0) \ge 1$, and $v$ will be matched deterministically to some neighbor $w$ of level -1.
The runtime of the call to $\setlvl(v,0)$  is $O(\phi_v(1) + O(\log n)) \cdot O(\log n) = O(\log^4 n)$ by Claim \ref{setlevelTime}.
Similarly, we have $\phi_w(1) = O(\log^3 n)$,  % by Invariant \ref{risei},
and the runtime of the call to  $\setlvl(w,0)$  is $O(\phi_w(1) + O(\log n)) \cdot O(\log n) = O(\log^4 n)$.  % by Claim \ref{setlevelTime}.
Since $w$ is of level -1, it was unmatched by Invariant \ref{1c}, so in this case the procedure does not proceed recursively.
Consequently, the time required by Procedure $\evalf$ to handle any level-0 vertex is $O(\log^4 n)$.


\subsubsection{Levels with $T_\ell / \Delta < 1$} \label{lowlevels}
In levels for which the simulation time is smaller than 1, the adversary does not make any update operation within the time required by a level-$\ell$ thread to complete its entire execution.
For such levels $\ell$ the queue $\cQ_\ell$ of temporarily free vertices is empty, and every level-$\ell$ vertex that becomes temporarily free is handled immediately by this procedure, i.e., without simulating the execution of this procedure over multiple update operations.
Note that the active vertices for such levels $\ell$ may constitute a significant part of $N_{\ell}(v)$, hence $N'_\ell(v)$ may be significantly smaller than $\gamma^\ell$,
meaning that the sample space will be too small.
However, for such levels there is no need for probabilistic arguments, as we may naively scan all vertices of $N'_\ell(v)$, match $v$ with an arbitrary free vertex $w$ there,
or leave $v$ free if none is found. In the former case we let $v$ and $w$ fall and rise to the same level $\ell$, respectively, by calling to $\setlvl(v,\ell)$ and $\setlvl(w,\ell)$, and then match $v$ with $w$, thus creating a new level-$\ell$ matched edge.
In the latter case $v$ remains free, and we make the call $\setlvl(v,-1)$.
The cost of this deterministic treatment is
%
dominated by other parts of this procedure. (Disregarding the calls  $\setlvl(v,\ell)$ and $\setlvl(w,\ell)$, this cost
is linear in the size of $N_{\ell}(v)$, which does not exceed  $\phi_v(\ell) = \gamma^{\ell} \cdot O(\log^2 n)$ by Invariant \ref{risei}.)

%We next analyze the runtime of Procedure $\evalf$.
%\begin{lemma}
%Denote by $H_\ell$ the maximum time needed for executing Procedure $\evalf(v)$, where $v$ ranges over all level-$\ell$ vertices.
%Then $H_\ell = O(\gamma^{\ell} \cdot \log^4 n)$.
%\end{lemma}
\subsubsection{Proof of Lemma \ref{evalftime}} \label{evalftimepf}
Consider an arbitrary level-$\ell$ vertex $v$ handled by Procedure $\evalf$.
By the detailed description of the procedure provided above,  the (overall) time needed for computing  the values $\phi_v(j)$ and vertex sets $N_v(j)$ (including the authentication process), for all   $j \le \ell_v$,
then computing the index $\ell$ and the vertex set $N'_v(\ell)$, next randomly sampling a random mate $w$ for $v$ and matching them,
and finally executing the calls $\setlvl(v,\ell)$ and $\setlvl(w,\ell)$, is $O(\gamma^{\ell} \cdot \log^4 n)$.
%As explained, above,  can be carried out in $O(\log n)$ time.
Since the level of the old mate $w'$ of $w$ (if exists) is at most $\ell-1$,
the time needed by the recursive call $\evalf(w')$ is bounded by $H_{\ell-1}$.
We thus obtain the recurrence $H_\ell \le O(\gamma^{\ell} \cdot \log^4 n) + H_{\ell-1}$.
Note that the basis of this recurrence is $H_0 = O(\log^4 n)$,  thus resolving to $H_\ell = O(\gamma^{\ell} \cdot \log^4 n)$. \QED
%\end{proof}

\subsection{The Behavior of Falling and Rising Vertices} \label{behavior}
Consider an arbitrary level-$\ell$ vertex $v$ handled by Procedure $\evalf$.
By the description of the procedure, $v$ falls from level $\ell^{(0)} := \ell_v$ to level $\tilde \ell^{(0)} := \ell$.
It is possible that $\ell^{(0)} = \tilde \ell^{(0)}$, in which case the level of $v$ remains unchanged.  % and we say that $v$ is \emph{stagnant}.
On the other hand, $w$ rises from level $\ell^{(1)} := \ell_w$ at most $\tilde \ell^{(0)}-1$ to level $\tilde \ell^{(0)}$.
Assuming $w$ was previously matched to $w'$, the matched edge $(w,w')$ gets deleted from the matching
and the edge $(v,w)$ is inserted to the matching instead, and the procedure proceeds recursively to handling $w'$.
By Invariant \ref{first}(b), the level of $w'$ is $\ell^{(1)}$.  %, and it now replaces the role of vertex $v$.
% the same as that of $w$, $\ell_w$, before it started rising.
%Write $\ell_v = \ell^{(0)}$ and $\ell_w = \ell^{(1)}$.
Therefore, in the first recursion level, a single vertex fell from level $\ell{(0)}$ to level $\tilde \ell^{(0)}$ (possibly $\ell^{(0)} = \tilde \ell^{(0)}$, but we
may view this too as a fall)
and a single vertex rose from level $\ell^{(1)} \le \tilde \ell^{(0)} -1$ to level $\tilde \ell^{(0)}$.
%While $v$ was temporarily free at the beginning of the execution, it becomes matched and at the expense
%Moreover, a single matched edge got deleted from the matching at level $\ell^{(1)}$.
The next lemma follows by a simple induction.
\begin{lemma} \label{parenthesis}
For each recursion level $i = 0,1,\ldots$, let $\ell^{(i)}$ denote the level of the vertex that the recursive call handles,
let $\tilde \ell^{(i)}$ denote the level to which that vertex falls in order to match,
and let $\ell^{(i+1)}$ be the (old) level of its new mate, which rises to level $\tilde \ell^{(i)}$ for the match.
Then for any $i$ and $j$ with $i < j$, we have
$$\ell^{(i)} ~\ge~ \tilde \ell^{(i)} ~>~   \ell^{(i+1)} ~\ge~ \ell^{(j)} ~\ge~ \tilde \ell^{(j)} ~>~ \ell^{(j+1)}.$$
In particular, as part of the execution of this procedure, at most $\log_\gamma(n-1)+1$ vertices are falling and at most $\log_\gamma(n-1)$ vertices are rising.
%For any level $\ell$, at most one vertex falls to level $\ell$ and another one rises to level $\ell$ throughout the execution of this procedure.
\end{lemma}
%[[S: changed]]

The description of Procedure $\evalf$ and Lemma \ref{parenthesis} yield the following corollaries.
\begin{corollary} \label{boundactive}
Among all   vertices that become temporarily free (and active) as part of the execution of Procedure $\evalf(v)$, at most three are temporarily free at any point in time during this execution.
\end{corollary}
%We say that a fall of a vertex $v$ \emph{intersects} level $\ell$ if it is from level at least $\ell$ to level lower than $\ell$.
\begin{corollary} \label{falling}
As part of the execution of Procedure $\evalf(v)$, vertices of level higher than $v$'s original level $\ell_v$ remain intact.
% and in particular, no such vertex falls.
For any   $\ell \le \ell_v$:
~(1) At most one vertex falls from level $\ge \ell$ to level $< \ell$.
~(2) At most one matched edge gets deleted at  level $\ell$; at most one matched edge gets created at level $\ell$. %; one of its endpoints rises to create a new matched edge.
%For each vertex that rises to create a new matched edge, its old matched edge (if exists) got deleted from the matching.
%This is the only matched edge that gets deleted at that level
%Hence, throughout the execution of this procedure, at most $\log_2(n-1)$ matched edges are deleted from the matching, each at a different level.
\end{corollary}
\begin{corollary} \label{threadeval}
The call to $\evalf(v)$ is executed by a thread of level at least $\ell_v$.
For any $\ell$, a thread must be of level at least $\ell$ to handle:
%$\ell$ if it is from level at least $\ell$ to level lower than $\ell$.
~(1) A vertex falling from level $\ge \ell$ to level $< \ell$ due to Procedure $\evalf$.  % is handled by a thread of level at least $\ell$.
~(2) A vertex rising to level $\ell$ due to Procedure $\evalf$.  % is handled by a thread of level at least $\ell$.
~(3) A level-$\ell$ matched edge that gets deleted due to Procedure $\evalf$.  % is handled by a thread of level at least $\ell$.
\end{corollary}





==> strengthen.tex <==

%[[S: till here]]
\section{Strengthening the algorithm of \cite{GP13}} \label{changes}
%The main goal of this section is to provide
%We achieve this goal, we provide by strengthening a scheme
Gupta and Peng \cite{GP13} presented a scheme for maintaining approximate matchings in dynamic graphs,
yielding algorithms for maintaining $(1+\eps)$-approximate matching with worst-case update times of $O(\sqrt{m} / \eps^2)$ and $O(\Delta / \eps^2)$ in general graphs
and graphs with degree bounded by $\Delta$, respectively.
The scheme of \cite{GP13} was refined in \cite{PS16} to provide a worst-case update time of $O(\alpha / \eps^2)$ for graphs with arboricity bounded by $\alpha$; since the arboricity of any $m$-edge graph is $O(\sqrt{m})$ and at most twice the maximum degree,
the result of \cite{PS16} generalizes that of \cite{GP13}.
The algorithm of \cite{GP13} for bounded degree graphs, applied for a degree bound of $O(m^{1/4} \sqrt{\eps})$, was used as a black-box to obtain an algorithm for maintaining $(3/2 + \eps)$-approximate matching with worst-case update time $O(m^{1/4}/\eps^{2.5})$ in bipartite graphs \cite{BS15}.
%, and then in general graphs \cite{BS16}.
The drawback of the scheme of \cite{GP13} is that the worst-case number of changes (replacements) to the maintained matching may be linear in the matching size, which could be significantly larger than the required worst-case update time.
Since the algorithms of \cite{GP13,BS15,PS16} follow this scheme, they all suffer from the same drawback.

In this section we demonstrate that the scheme of \cite{GP13} can be strengthened to guarantee that the number of matching replacements is the same as the update time (up to a small constant), also in the worst-case. The resulting stronger version of the scheme of \cite{GP13}, applied in the particular case of constant degree graphs, was already used in Section \ref{sec:almost} to derive a polylogarithmic worst-case bound on the number of replacements to the matching guaranteed by Theorem \ref{maint} (see the second remark following Theorem \ref{maint}).
%(Aiming for conciseness, we provide here  only a sketch of the argument; refer to \cite{Sol17} for a more elaborate argument.)
Moreover, as an immediate corollary of this stronger scheme, the algorithms of \cite{GP13,BS15,PS16} are strengthened in the same way, i.e., so as to guarantee that the worst-case number of replacements in the corresponding matchings is asymptotically the same as the worst-case update time.


\subsection{The amortization scheme of \cite{GP13}} \label{amor}
The scheme of \cite{GP13} exploits a basic \emph{stability} property of matchings: The size of the maximum matching changes by at most 1 following each update.
Thus if we have a \emph{large} matching  of size close to the maximum,
%If the size $|\cM^*|$ of the maximum matching is large and we have a matching $\cM$ whose size is close to $|\cM^*|$,
 it will remain close to it throughout a long update sequence, or formally:
  \begin{lemma} [{\bf Lemma 3.1 in \cite{GP13}}] \label{lazylemma}
%\vspace{-5pt} [Proof in Appendix \ref{app:lazy}]}
Let $\eps,\eps' \le 1/2$. Suppose that $\cM_i$ is a $(1+\eps)$-approximate matching for $G_i$.
For $j = i,i+1,\ldots, i+\lfloor \eps'\cdot |\cM_i| \rfloor$, let $\cM^{(j)}_i$ denote the matching $\cM_i$ after removing from it all edges that got deleted during the updates $i+1,\ldots,j$.
Then $\cM^{(j)}_i$ is a $(1+2\eps+2\eps')$-approximate matching for the graph $G_j$.
\end{lemma}
We remark that Lemma \ref{lazylemma} can be easily generalized, so that if $\cM_i$ is a $(t+\eps)$-approximate matching for $G_i$, for any $t \ge 1$,
then $\cM^{(j)}_i$ is a $(t(1+2\eps')+2\eps+2\eps')$-approximate matching for  $G_j$, for any $j$. 
(For $t = 1$ this gives rise to an approximation of $1 +2\eps + 4\eps'$, which is slightly worse than the $(1+2\eps+2\eps')$-approximation of Lemma \ref{lazylemma}.)
For clarify of presentation, we consider the regime of approximation guarantee $1+\eps$ in the sequel. However,   the same argument works for any approximation guarantee.

Hence, one can compute a $(1+\eps/4)$-approximate matching $\cM_i$ at a certain update $i$, and use the same  matching $\cM^{(j)}_i$ throughout all updates $j = i,i+1,\ldots, i' =  i+ \lfloor \eps/4\cdot |\cM_i| \rfloor$. (By Lemma \ref{lazylemma}, $\cM^{(j)}_i$ is a $(1+\eps)$-approximate matching for all graphs $G_j$.)
%throughout these updates the original matching $\cM_i$ (minus edges that might be deleted from it during this time)
%continues to provide a $(1+O(\eps))$-MCM, with a larger constant hiding in the $O$-notation.
Next compute a fresh $(1+\eps/4)$-approximate matching $\cM_{i'}$ following update $i'$ and use it throughout all updates $i',i'+1,\ldots,i'+ \lfloor \eps/4 \cdot |\cM_{i'}|\rfloor$, and repeat.

In this way the static time complexity of computing a $(1+\eps)$-approximate matching $\cM$
%\cite{HK73,MV80,Vaz12},
is \emph{amortized} over $1 + \lfloor \eps/4\cdot |\cM| \rfloor  = \Omega(\eps \cdot |\cM|)$ updates.
The key insight behind the scheme of \cite{GP13} (which was refined in \cite{PS16}) is not to compute the approximate matching on the entire graph $G$, but rather on a \emph{matching sparsifier}, which is a sparse subgraph $\tilde G$ of  $G$ which preserves (or approximates to within a factor of $1+\eps$, as in \cite{PS16})
the maximum matching size.
The matching sparsifier of \cite{GP13, PS16} is derived from a constant approximate vertex cover that is maintained dynamically \emph{by other means}.
For brevity, we shall not describe here how a vertex cover is maintained or how the sparsifier is computed on top of it; the interested reader can refer to \cite{GP13,PS16} for details. The bottom-line of \cite{PS16} is that for graphs $G$ with arboricity bounded by $\alpha$, for any $1 \le \alpha = O(\sqrt{m})$,
%: (1) a constant-approximate vertex cover can be maintained with a worst-case update time of $O(\alpha / \eps)$, and (2)
the matching sparsifier $\tilde G$   has $O(|\cM| \cdot \alpha/\eps)$ edges, and it can be computed in time linear in its size.
(The scheme of \cite{PS16} generalizes that of \cite{GP13}, hence we may restrict attention to it.)
A $(1+O(\eps))$-approximate matching can be computed for the sparsifier $\tilde G$ in time $O(|\tilde G| / \eps) = O(|\cM| \cdot \alpha/\eps^2)$ \cite{HK73,MV80,Vaz12},
and assuming the constant hiding in the $O$-notation is sufficiently small, it provides a $(1+\eps/4)$-approximate matching for the entire graph.
Since the cost $O(|\cM| \cdot \alpha/\eps^2)$ of this static computation is amortized over  $\Omega(\eps \cdot |\cM|)$ updates,
the resulting amortized update time is $O(\alpha \cdot \eps^{-3})$. (One can shave a $1/\eps$-factor from this bound, but we ignore this minor improvement.)

\subsection{A Worst-Case Bound}
The amortization scheme of Section \ref{amor} computes a $(1+\eps/4)$-approximate matching $\cM$ \emph{from scratch}, and then re-uses it throughout $1+\lfloor \eps/4 \cdot |\cM| \rfloor$ additional updates. The worst-case update time is thus the static computation time of an approximate matching, namely, $O(|\cM| \cdot \alpha/\eps^2)$.
To improve the worst-case guarantee, the trick used in \cite{GP13,PS16} is to simulate the static   matching computation within
a ``window'' of $1+\lfloor \eps/4 \cdot |\cM| \rfloor$  consecutive updates, so that following each update the algorithm simulates only
$O(|\cM| \cdot \alpha/\eps^2) / (1+\lfloor \eps/4 \cdot |\cM| \rfloor = O(\alpha \cdot \eps^{-3})$
%$O(\min\{m,|\cM|^2\}/\eps)/(1+\lfloor \eps/4 \cdot |\cM| \rfloor) = O(\sqrt{m} \cdot \eps^{-2})$
steps of the static computation.
During this   window the gradually-computed matching $\cM'$ is useless, so the previously-computed matching $\cM$ is re-used as the output matching.
This means that each matching is re-used throughout a time window of twice
as many updates, hence the approximation guarantee increases from $1+\eps$ to $1+2\eps$.
%(We allow the approximation guarantee to grow from $1+\eps$ to $1+O(\eps)$, since we can reduce it back to $1+\eps$ by scaling.)
%{[[S: A remark that may confuse the reader:
Clearly, the gradually-computed matching does not include edges that got deleted from the graph during the window.

Although this tweak guarantees a worst-case update time of $O(\alpha \cdot \eps^{-3})$, the number of replacements may be huge in the worst-case.
Indeed, once the computation of $\cM'$ ends, the output matching is switched from the old matching $\cM$ to the new one $\cM'$ \emph{instantaneously}, which may require $|\cM| + |\cM'|$ replacements to the output matching at that time. To bound the number of replacements in the worst-case, we an additional   window of $W = \Theta(\eps \cdot |\cM|)$ updates, during which we gradually transform $\cM$ into $\cM'$ until both matchings coincide, performing $O(\alpha \cdot \eps^{-1})$ replacements following every update step.

Next, we describe this gradual transformation process.

Let $t$ and $t' = t + W$ denote the update steps in which this transformation process starts and ends, respectively.
We refer to the matching that we output throughout this process as the \emph{source matching}, and denote it by $\cM^*_{i}$, for $i = t, t+1, \ldots, t'$;
the source matching coincides with $\cM$ initially, i.e., $\cM^*_t = \cM$,
 and is gradually transformed into the \emph{target matching} $\cM'_{i}$,
 until coinciding with it at (or before) step $t'$, i.e., $\cM^*_{t'} = \cM'_{t'}$.
 The target matching $\cM'_i$ coincides with $\cM'$ initially, i.e., $\cM'_t = \cM'$,
 but may gradually deviate from it due to edge deletions; for a general $i = t, t+1, \ldots, t'$, $\cM'_i$ is obtained from $\cM'$ by removing from it all edges that got deleted from the graph between steps $t$ and $i$.
%Denote by $\cM_i$ the matching obtained from $\cM$ and
The source matching $\cM^*_i$ is different than the \emph{old matching} $\cM_i$, i.e., the matching obtained from $\cM$ by removing from it all edges that got deleted from the graph between steps $t$ and $i$, hence the need for this additional notation.
%Similarly to $\cM_i$, the target matching $\cM'_{i}$ may change over time due to edges that are deleted from the graph during the transformation process,
%but no other changes are made to $\cM'_{i}$,
%i.e., $\cM'_i$ is obtained from $\cM'$ after removing from it all edges that got deleted until step $i$.  % during the transformation process.

We say that an edge of $\cM'_{i} \setminus \cM^*_i$ that is incident on at most one edge of $\cM^*_i$ is \emph{safe}, otherwise it is \emph{risky}, being incident on two edges of $\cM^*_i$.  Since $\cM^*_i$ serves as our output matching throughout the transformation process, it has to be a valid matching all along the process,
which implies that adding a risky edge to $\cM^*_i$ must trigger
%Adding a safe edge to $\cM_i$ triggers the deletion of at most one edge of $\cM_i$.
%The first thing to note is that we cannot add arbitrary edges of $\cM'_{i} \setminus \cM_i$ to $\cM_i$.
the deletion of two edges from $\cM^*_i$.
Thus if we keep adding risky edges to $\cM^*_i$, the approximation guarantee of the source matching (which is our output matching) may double throughout the transformation process.
%Although we sometimes have to add risky edges for the transformation process to proceed,
The following lemma shows that if all edges of $\cM'_{i} \setminus \cM^*_i$ are risky, the source matching is just as large as the target matching.
%, in which case we can afford to slightly hurt the approximation guarantee by adding a risky edge and deleting two edges as a result.
\begin{lemma} \label{riskyedge}
If all edges of $\cM'_{i} \setminus \cM^*_i$ are risky, then $|\cM^*_i| \ge |\cM'_i|$.
\end{lemma}
\begin{proof}
%We assume all edges in $\cM'_{i} \setminus \cM_i$ are risky, and show that $|\cM_i| \ge |\cM'_i|$.
Consider a bipartite graph $L \cup R$, where each vertex in $L$ corresponds to an edge of $\cM'_{i} \setminus \cM^*_i$
and each vertex in $R$ corresponds to an edge of $\cM^*_{i} \setminus \cM'_i$, and there is an edge between a vertex in $L$ and a vertex in $R$ iff the corresponding matched edges share a common vertex in the original graph.
% and show an injection from $S' = \cM'_{i} \setminus \cM_i$ to $S = \cM_{i} \setminus \cM'_i$.
If all edges of $\cM'_{i} \setminus \cM^*_i$ are risky, then any edge of $\cM'_{i} \setminus \cM^*_i$ is incident on two edges of $\cM^*_i$, and since $\cM'_i$ is a valid matching,
those two edges cannot be in $\cM'_i$. In other words, the degree of each vertex in $L$ is exactly 2.
Also, the degree of each vertex in $R$ is at most 2, as $\cM'_i$ is a valid matching.
 It follows that $|R| \ge |L|$, or in other words $|\cM^*_{i} \setminus \cM'_i| \ge |\cM'_{i} \setminus \cM^*_i|$, yielding $|\cM^*_i| \ge |\cM'_i|$.
\QED
\end{proof}

The transformation process is carried out as follows. The sliding window of length $W = \Theta(\eps \cdot |\cM|)$ is halved into two smaller windows.
The sets of safe and risky edges in $\cM'_t \setminus \cM^*_t$ can be computed within time $O(|\cM| + |\cM'|) = O(|\cM|)$ in the obvious way,
and we can thus gradually simulate this static computation over the $W/2$ update steps of the first window, performing 
$O(|\cM|) / (W/2) = O(\alpha \cdot \eps^{-1})$ computational steps following each update.
Moreover, following each edge deletion from the graph, we can update the sets of safe and risky edges in  $\cM'_i \setminus \cM^*_i$
in constant time, where $i$ is the corresponding update step.
We may henceforth assume that the sets of safe and risky edges in $\cM'_{t+W/2} \setminus \cM^*_{t+W/2}$
are fully up-to-date at the start of the second window, and we continue to maintain them throughout this window.
(Note also that at the start of the second window, the source matching coincides with the old matching, i.e., $\cM^*_{t+W/2} = \cM_{t+W/2}$, since we did not make any changes to it throughout the first window.)
At every update step of the second window $i = t + W/2, t+W/2 + 1, \ldots,t'$, we add $O(\alpha \cdot \eps^{-1})$ edges of $\cM'_i \setminus \cM^*_i$ (if any) to $\cM^*_i$, by giving precedence to safe edges, i.e., adding risky edges to $\cM^*_i$ only when there are no safe edges to add. Following every such addition,
we delete the at most two edges in $\cM^*_i$ incident on the newly added edge (if any), and update the sets of safe and risky edges in $\cM'_i \setminus \cM^*_i$ in constant time.
%(One may argue that the notation $\cM^*_i$ is not well-defined, as this matching changes multiple times following the $i$th update step.
%Since we add and delete multiple edges to and from $\cM^*_i$ following the $i$th update step, and we
%Although the matching that we output as $\cM^*_i$ is the one resulting at the end of this process,
(Although $\cM^*_i$ is gradually updated by those $O(\alpha \cdot \eps^{-1})$ edge additions and deletions,
we may use the same notation $\cM^*_i$ to refer to any of the matchings obtained along this gradual update.)

This transformation process clearly guarantees that the number of replacements made to the output matching is bounded by $O(\alpha \cdot \eps^{-1})$
in the worst-case.
Since we add $O(\alpha \cdot \eps^{-1})$ edges of $\cM'_i \setminus \cM^*_i$ to $\cM^*_i$
following every update step of the second window in which $\cM'_i \setminus \cM^*_i$ is non-empty and as $W/2 = \Theta(\eps \cdot |\cM|) = \Omega(\eps \cdot |\cM'_i \setminus \cM^*_i|)$, 
$\cM'_i \setminus \cM^*_i$ must become empty well before the end of that window.
%Consequently, before the end of the process, 
At that time the output matching must contain the target matching. 
Of course, we can also guarantee that these matchings coincide, by gradually deleting edges of $\cM^*_i \setminus \cM'_i$ from $\cM^*_i$ 
throughout an additional window of $W$ updates,
%following every update step in which $|\cM^*_i| \ge |\cM'_i|$, 
but it is actually only better to end this process with a larger matching than needed.
Once the transformation process ends, we start a new one, and repeat.
To conclude the argument, we argue that the output matching $\cM^*_i$ is a valid $(1+O(\eps))$-approximate matching, for any $i, t \le i \le t'$.
%We first argue that the output matching $\cM^*_i$ is a valid matching. Indeed,
In the first window of length $W/2$   the output matching coincides with the old matching $\cM_i$,
which is a $(1+O(\eps))$-approximate matching by Lemma \ref{lazylemma}. It is left to prove the following lemma.
%we may henceforth consider just the second window.
%
%The following lemma
%To conclude the argument we employ the following lemma.
%Denote by $\cM_i$ the matching obtained from $\cM$ after removing from it all edges that got deleted from the graph between steps $t$ and $i$, for $i = t, t+1, \ldots, t'$.
\begin{lemma}
$\cM^*_i$ is a valid $(1+O(\eps))$-approximate matching, for any $i = t + W/2, t+W/2 + 1, \ldots,t'$.
\end{lemma}
\begin{proof}
It is immediate that the output matching $\cM^*_i$ is a valid matching, for any $i = t + W/2, t+W/2 + 1, \ldots,t'$,
as we proactively delete from it edges that share a common vertex with new edges added to it.
%guarantee that no two edges of the output matching share a common vertex by deleting edges
%following every edge addition to the output matching throughout the en second window.

Fix any  $i \in \{t + W/2, t+W/2 + 1, \ldots,t'\}$. We next analyze the approximation guarantee of $\cM^*_i$.

Suppose first that we add only safe edges to the output matching between update steps $t+W/2$ and $i$.
Every safe addition to the output matching triggers at most one deletion from it.
%In this case every newly added edge to the output matching triggers the deletion of at most one edge from it,
Recalling that $\cM^*_{t+W/2} = \cM_{t+W/2}$, we conclude that the size of the output matching cannot be smaller than that of the old matching by more than $W/2$, which upper bounds the number of edges deleted from the graph in the entire second window, and in particular until update step $i$, thus we have $|\cM^*_i| \ge |\cM_i| - W/2$.

We henceforth assume that at least one risky edge is added to the output matching between steps $t+W/2$ and $i$, and let $j$ be the last step when such an addition occurs.
Just before this addition, we have $|\cM^*_j| \ge |\cM'_j|$ by Lemma \ref{riskyedge}, thus we have
$|\cM^*_j| \ge |\cM'_j| - 1$ after adding that risky edge to $\cM^*_j$ and deleting the two edges incident on it.
At any subsequent moment in time until update step $i$, only safe edges are added to the output matching,
hence its size cannot be smaller than that of the target matching by more than $W/2 + 1$, thus we have $|\cM^*_i| \ge |\cM'_i| - W/2 - 1$.

We have shown that $|\cM^*_i| \ge \min\{|\cM_i|,|\cM'_i|\} - W/2 - 1$.
By Lemma \ref{lazylemma}, both $\cM_i$ and $\cM'_i$ are $(1+O(\eps))$-approximate matchings.
It follows that $ |\cM| \le (1 + O(\eps)) \cdot \min\{|\cM_i|, |\cM'_i|\}$, hence $W = \Theta(\eps \cdot |\cM|) = O(\eps \cdot \min\{|\cM_i|,|\cM'_i|\})$,
which completes the proof of the lemma.
\QED
\end{proof} 
